Airy structures and deformations of curves in surfaces

An embedded curve in a symplectic surface $\Sigma\subset X$ defines a smooth deformation space $\mathcal{B}$ of nearby embedded curves. A key idea of Kontsevich and Soibelman arXiv:1701.09137 [math.AG], is to equip the symplectic surface $X$ with a foliation in order to study the deformation space $\mathcal{B}$. The foliation, together with a vector space $V_\Sigma$ of meromorphic differentials on $\Sigma$, endows an embedded curve $\Sigma$ with the structure of the initial data of topological recursion, which defines a collection of symmetric tensors on $V_\Sigma$. Kontsevich and Soibelman define an Airy structure on $V_\Sigma$ to be a formal quadratic Lagrangian $\mathcal{L}\subset T^*(V_\Sigma^*)$ which leads to an alternative construction of the tensors of topological recursion. In this paper we produce a formal series $\theta$ on $\mathcal{B}$ of meromorphic differentials on $\Sigma$ which takes it values in $\mathcal{L}$, and use this to produce the Donagi-Markman cubic from a natural cubic tensor on $V_\Sigma$, giving a generalisation of a result of Baraglia and Huang, arXiv:1707.04975 [math.DG].

==> K3.tex <==
\subsubsection{Elliptic fibrations}

A rich class of examples arise from Elliptic fibrations of K3 surfaces. 
Recall that a K3 surface is called elliptic when there is a surjective morphism $\pi: X \rightarrow \bp^1$ whose generic fiber is a smooth curve of genus one.
A generic K3 surface is not elliptic and they form a dense codimension one subset of the moduli space of complex K3 surfaces.
Such morphisms are always flat and therefore all fibers have arithmetic genus one. The simplest class of elliptic surfaces are obtained from Kummer surfaces of the form $X=E_1 \times E_2$, where $E_1$ and $E_2$ are elliptic curves. Two special fibrations are obtained via the projections of the surface $X$ to the quotients $E_i/\iota \cong \bp^1$, where $\iota$ is the elliptic involution on the curve. Elliptic surfaces with a section are described by their Weierestras form:
$$\fy^2=\fz^3+f(\fx)\fz+g(\fx),$$
where $\fx,\fy,\fz$ are local coordinates and $f(\fx), g(\fx)$ are polynomials of $\deg f=8, \deg g=12$. Any such surface is foliated by fibers of the elliptic fibration. 
We equip the surface $X$ with the symplectic form 
$$\omega=\frac{d\fz \wedge d\fx}{\fy}.$$
There is a construction of an algebraically completely integrable Hamiltonian system associated to K3 surfaces and a linear system due to Beauville \cite{beauville1991systemes}. There are two realizations of this integrable system: the first one is based on a linear system $|D|$ of curves of genus $g$ on the surface. The resulting integrable system is a Lagrangian fibration $\pi:\cj \rightarrow |D|=\bp^g$, where any point $b \in \bp^g$ corresponds to a curve in the linear system and fibers of $\pi$ are compactified Jacobians of degree $g$ divisors on such curves.
In the following we restrict to the open subset $B \subset \bp^g$ corresponding to smooth curves and denote the restricted Lagrangian fibration by the same letter.
There is another realization of this integrable system in terms of the symmetric products $X^{(g)}=\mathrm{Sym}^g (X)$ of the K3 surface $X$: if we take $g$ generic points $\{p_1, \dots, p_g\}$ of $X$ we obtain a hyperplane $H \subset \bp^g$ passing through these points (Here we use the linear system to define an embedding $X \rightarrow \bp^g$ and therefore we think of $X$ as a subset of $\bp^g$ using this embedding). This gives a curve $C=X \cap H$ containing the points $p_1,\dots,p_g$ and we obtain a map
$$(p_1,\dots,p_g) \mapsto ([C], [p_1+\dots + p_g]).$$
Notice that both realizations give symplectic manifolds: the first realization can be identified with the moduli space of sheaves which has a symplectic structure by \cite{mukai1984symplectic} and the symplectic strcture on the symmetric product $X^{(g)}$ is induced from the symplectic structure of the K3 surface $X$. One of the results of Beauville is that the identification above preserves the symplectic structure.

Here we study an example coming from hyperelliptic curves on such K3 surfaces based on the article \cite{takasaki2001hyperelliptic}.
We first define a five dimensional family of curves $C_b$ for $b=(\z_1, \dots ,\z_5)$ given by the equation
$$z=P(\fx)=\sum_{i=1}^5 \z_i \fx^{5-i},$$
which defines a family of hyperelliptic curves of genus 5 defined by the equation
$$\fy^2=P(\fx)^3+f(\fx)P(\fx)+g(\fx).$$
Such curves can be identified with hyperplane sections of the following finite morphism 
$$\phi: X \rightarrow \bp^5 \qquad (\fx,\fy,\fz) \mapsto (-\fz:\fx^4:\fx^3:\fx^2:\fx:1).$$
There is a map from the symmetric product $X^{(5)}$ to $B$ defined as follows: for a given collection $\{p_1, \dots, p_5\}$ of 5 points on $X$ with $p_i=(\fx_i,\fy_i,\fz_i)$ and a point $b \in B$ the curve $C_b$ passes through these points when the conditions $P(\fx_i)=\fz_i$ are satisfied for $i=1,\dots,5$. These conditions are equivalent to the identity:
$$P(\fx)=\sum_{i=1}^5 \fz_i \prod_{j \neq i} \frac{\fx-\fx_j}{\fx_i-\fx_j}.$$
This specifies the local coordinates $\z_i$'s on the space $B$ in terms of $x_i,z_i$'s and defines the desired function $X^{(5)} \rightarrow B$. 
Beauville \cite{beauville1991systemes} identified the symplectic structure on $X^{(5)}$ given by
$$\Omega=\sum_{i=1}^5 \frac{d\fz_i \wedge d\fx_i}{\fy_i}$$
with the symplectic structure on the relative Picard scheme over $B$.

Beauville's construction is using the relative Picard scheme. 
Here we consider the Jacobian varieties instead and the relative Jacobian $\cj \rightarrow B$ whose fiber at the point $b \in B$ is the Jacobian of degree zero divisors on the curve $C_b$.
We work the following basis of holomorphic differentials:
$$\omega_i=\frac{\fx^{5-i} d\fx}{\fy}, \quad i=1,\dots,5.$$
The Abel-Jacobi map in terms of this choice of basis is defined as
$$(p_1, \dots,p_5) \rightarrow (\w_1,\dots,\w_5),$$
where
$$\w_i=\sum_{j=1}^5 \int_{(\infty,\infty)}^{(\fx_j,\fy_j)} \omega_i.$$
The collection $\z_1,\dots,\z_5,\w_1,\dots,\w_5$ gives local coordinates on the relative Jacobian $\cj$. In \cite{takasaki2001hyperelliptic} it is proved that the following relations hold:
$$\frac{\partial \w_i}{\partial \z_j}=\frac{\partial \w_j}{\partial \z_i},$$
and therefore we can define a locally defined holomorphic function $F$ such that $\w_i=\frac{\partial F}{\partial \z_i}$.
Furthermore, the symplectic form with respect to the coordinates $\z_i,\w_i$ has the following form:
$$\omega=\sum_{i=1}^5 d\z_i \wedge d \w_i.$$

\subsubsection{The Beauville-Mukai integrable system}

In this section we consider a polarized K3 surface $(X,H)$ and study an associated integrable system corresponding to a moduli space of sheaves on the surface. 
Recall that the support, \( \mathrm{Supp}\), of a coherent sheaf $\fF$ is defined as
$$\mathrm{Supp}(\fF)=\{x: \fF_x \neq 0\}.$$
The dimension of a sheaf is defined as the dimension of its support.
We say that a sheaf $\fF$ is pure if for every non-trivial subsheaf $\fG \subset \fF$ we have the equality $\dim \fG=\dim \fF$.
In the following we will be interested in one dimensional sheaves on the surface.
After fixing a polarization $H$ on $X$, which is an ample and primitive divisor, we define the twisted sheaf $\fF(m)$ as the tensor product $\fF \otimes \co_X(m H)$ associated with any integer $m$. The Hilbert polynomial of $\fF$ with respect to the polarization $H$ is defined as $P_\fF(m)=\chi(\fF(m))$ and it can be written as
$$P_\fF(m)=\sum_{k=0}^{\dim \fF} \alpha_k(\fF) \frac{m^k}{k!}.$$
The reduced Hilbert polynomial of $\fF$ is defined as
$$p_\fF(m)=\frac{P_\fF(m)}{\alpha_{\dim \fF}(\fF)}.$$
The rank of the sheaf $\fF$ is defined as 
$$\mathrm{rank}(\fF)=\frac{\alpha_{\dim X}(\fF)}{\alpha_{\dim X}(\co_X)}.$$
A non-tirival pure coherent sheaf $\fF$ is called semistable with respect to the polarization $H$ when for every non-trivial subsheaf $\fG \subset \fF$ we have
$$p_\fG(m) \leq p_\fF(m), \qquad \mathrm{for \ all \ large} \ m.$$
Furthermore, the sheaf $\fF$ is called $H$ stable if we have strict inequality for $m \geq 0$.

Consider the Mukai lattice 
$$H^\bullet(X)=H^0(X,\bz) \oplus H^2(X,\bz) \oplus H^4(X,\bz)$$
associated with a projective K3 surface $X$. It is equipped with the bilinear form
$$(v,w)=\int_X v_2 \wedge w_2- v_0 \wedge w_4+v_4 \wedge w_0,$$
where $v_i,w_i \in H^i(X,\bz)$ are components of $v$ and $w$.
The Mukai lattice is an even unimodular of rank 24 together with an isometric map
$$H^2(X,\bz) \oplus U = E_8(-1)^{\oplus 2} \oplus U^{\oplus 4},$$
where $E_8(-1)$ is the negative definite root lattice of type $E_8$ and $U$ is the unimodular hyperbolic lattice of rank two. 
To a coherent sheaf $\fF$ there is an associated Mukai vector $v(\fF)=ch(\fF) \sqrt{td(X)}$ in the Mukai lattice of $X$ which is the same as 
$$v(\fF)=(\mathrm{rank}(\fF),c_1(\fF), \chi(\fF)-\mathrm{rank}(\fF)).$$
Associated to every Mukai vector $v$ there is a locally finite countable system of hyperplanes in the real ample cone of the surface which are known as \emph{$v$-walls}. A polarization $H$ on the surface $X$ is called \emph{$v$-generic} when it belongs to the complement of $v$-walls.
For a given Mukai vector $v$ and a $v$-generic ample divisor $H$ there is a moduli space $M_H^s(v)$ corresponding to $H$-stable pure coherent sheaves $\fF$ on $X$ satisfying $v(\fF)=v$. In \cite{mukai1984symplectic} it is proved that the moduli space admits a holomorphic symplectic structure. The moduli space of stable sheaves is smooth of dimension $2+(v,v)$. 
If $v$ is a primitive Mukai vector and $H$ is a $v$-generic polarization then every $H$-semistable sheaf if $H$-stable and therefore the moduli space $M_H(v)$ is a projective and holomorhic symplectic manifold.
Deformation theory of the moduli space is controlled by the groups $\mathrm{Ext}^i$. 
More precisely, the Zariski tangent space at the moduli point $[\fF]$ is identified with $\mathrm{Ext}^1(\fF,\fF)$ and furthermore $[\fF]$ is a smooth point of $M_H(v)$ if the kernel of $\mathrm{tr}^2_\fF$ vanishes, where
$$\mathrm{tr}^2_\fF: \mathrm{Ext}^2(\fF,\fF) \rightarrow H^2(X,\co_X)$$
is the trace map induced from the natural map $\mathrm{tr}_\fF: \mathcal{H}om(\fF,\fF) \rightarrow \co_X$.



\begin{thm}[Mukai \cite{mukai1984symplectic}]
The moduli space of stable sheaves carries a holomorphic symplectic form $\omega$, which is for $\alpha,\beta \in T_{M_H(v),\fF}=\mathrm{Ext}^1(\fF,\fF)$ given by
$$\omega(\alpha,\beta)=\int_X \omega_X \wedge \mathrm{tr}^2_\fF (\alpha \cup \beta),$$
where $\omega_X$ denotes a fixed holomorphic symplectic form on $X$.
\end{thm}
Every pure sheaf $\fF$ of dimension one on a smooth projective surface $X$ admits a locally free resolution
$$0 \rightarrow \fF_1 \xrightarrow{f}
 \fF_0 \rightarrow \fF \rightarrow 0$$
of length one such that $\fF_0$ and $\fF_1$ have the same rank $r$. The \emph{fitting support}, \( \mathrm{supp}\), of the sheaf $\fF$ is defined as the vanishing scheme of the induced morphism
$$\mathrm{supp}(\fF)=V(\wedge^r f)= V(\det f) \subset X.$$
\begin{example}
A particular class of such sheaves come from curves on the K3 surface $X$. More precisely, if a smooth curve $C$ of genus $g$ is the support of a sheaf $\fF$ with $rank(\fF|_C)=1$ and $\deg(\fF|_C)=k$ then the Mukai vector of $\fF$ is $(0,C,1-g+k)$.
\end{example}

Now take any primitive Mukai vector $v$ on $V$ of the form $v=(0,c_1(D),s)$ for a big and nef divisor $D$ on $X$ and assume that $(D,D)=2n-2$. This implies that the vector space $H^0(X,D)$ has dimension $n+1$ and therefore we obtain a morphism
$$\pi: M_H(v) \rightarrow |D|, \qquad \fF \rightarrow \mathrm{supp} (\fF).$$
This morphism is known to be a Lagrangian fibration and is called a Beauville-Mukai integrable system of $K3^{[n]}$-type. While the construction seems very restrictive it is conjectured that all Lagrangian fibrations by Jacobians are Beauville-Mukai systems.

\subsubsection{The connection between the Hitchin system and Beauville-Mukai system}

In \cite{sawon2019lagrangian} it was asked whether we can compute the Donagi-Markman cubic and special K\"ahler metric on the compactified Jacobian using topological recursion. The work of Donagi Ein Lazarsfeld describes the connection between the Hitchin system and the Beauville-Mukai system:

\begin{thm}[Donagi-Ein-Lazarsfeld \cite{donagi1997nilpotent}]
The Beauville-Mukai system built from $|NC|$ gives a compactification $\overline{M}_{GL}$ of the $GL(N,\bc)$-Hitchin system on $C$.
\end{thm}

Here is a brief description of the compactification of the Hitchin system: Denote by $\bk_C$ the compactification $\bp(K_C+\co_C)$ of the cotangent bundle of the curve $C$. We can view the curve $C$ as the zero section of the cotangent bundle $C \subset K_C \subset \bk_C$. Every spectral curve $\Sigma \subset \bk_C$ belongs to the linear system $\overline{B}=|NC|=\bp^g$, where $g=N^2(g_C-1)+1$.
The open subset $B \subset \overline{B}$ is defined as the set of curves not passing through the vertex of $\bk$. According to a result of Simpson \cite{simpson1994moduli} there is a projective moduli space 
$\overline{\ch}^k_{|NC|}$ parameterizing isomorphism classes of pairs of the form $(\Sigma, \fF)$ for curves $\Sigma \in |NC|$ and semi-stable coherent sheaves $\fF$ supported on $\Sigma$ with the same Hilbert polynomial as a line bundle of degree $k$ on a smooth member of the linear system $|NC|$.
This moduli space is equipped with the support map
$$\pi:\overline{\ch}^k_{|NC|} \rightarrow \overline{B}.$$
The Hitchin moduli space can be realized as an open subset of $\pi^{-1}(B)$ and the Hitchin map is the restriction of $\pi$ to this open subset. 
Now if we have a curve $C$ in the K3 surface $X$ defining an ample divisor consider the embedding
$$X \rightarrow \bp(H^0(X,\co_X(C))^*)=\bp^h.$$
If we take the cone inside $\bp^{h+1}$ over the K3 surface $X$ and intersect it with the pencil of hyperplanes in $\bp^{N+1}$ containing the curve $C$ we obtain a pencil of surfaces $X_t \rightarrow \bp^1$ such that every surface in this pencil contains a curve isomorphic to $C$. 
Curves in the linear system $|NC|$ in one of the K3 surfaces $X_t$ for $t \neq 0$ will deform to spectral curves in $X_0$.
Now the moduli space $\overline{\ch}^k_{|NC|}$ is fibered over $\bp^1$. The result of Donagi-Ein-Lazarsfeld says that fibers of the resulting fibration over $\bp^1$ are Beauville-Mukai systems on $X_t$ when $t \neq 0$ and the compactification of the GL-Hitchin system when $t=0$.

\subsubsection{Prepotential on the Beauville-Mukai system}
  
Recall that an \emph{algebraic integrable system} is a holomorphic map $\pi:X \rightarrow B$ where
\begin{enumerate}
    \item $(X,\omega)$ defines a complex holomorphic symplectic manifold.
    \item Fibers of the map $\pi$ are compact Lagrangian submanifolds.
    \item
    There is a smooth family of cohomology classes inside $H^{1,1}(X_b) \cap H^2(X_b,\bz)$ defining a positive polarization of the fiber $X_b$ for $b \in B$.
\end{enumerate}
  
\begin{thm}[Freed, Hitchin]
The space $B_{reg}$ admits a special K\"ahler metric of the form
$$\omega=-\frac{i}{2} \mathrm{Im}(\tau_{ij}) dz^i \wedge dz^j,$$
where $\tau_{ij}$ denotes the periods of the fibers.
\end{thm}

Consider the K\"ahler form $\omega$ on $B_{reg}$ and choose a collection of Darboux coordinates such that
$$\omega=\sum dx^i \wedge dy_i.$$
Denote $\pi^{(1,0)} \in \Omega^{1,0}(T_\bc)$ to be the projection onto the $(1,0)$ part of the complexified tangent bundle, then it can be written as 
$$\pi^{(1,0)}=\frac{1}{2} \left(dz^i \otimes \frac{\partial}{\partial x^i}-d\w_j \otimes \frac{\partial}{\partial y_j}\right),$$
for holomorphic functions $z^i,\w_j$. This equation implies that
$$\mathrm{Re}(dz^i)=dx^i, \qquad \mathrm{Re}(d\w_j)=-dy_j.$$
For any such Lagrangian fibration there is a locally defined holomorphic function $\cf$, well defined up to a constant, such that
$$\w_i=\frac{\partial \cf}{\partial z^j}, \qquad \tau_{ij}=\frac{\partial^2 \cf}{\partial z^i \partial z^j}.$$
This holomorphic function is called the prepotential associated with the special K\"ahler structure.

We can also write the K\"ahler form in terms of the prepotential:
$$\omega=\frac{i}{2} \mathrm{Im} \left(\frac{\partial^2 \cf}{\partial z^i \partial z^j} \right) dz^i \wedge d\overline{z^j}=\frac{i}{2} \mathrm{Im}(\tau_{ij}) dz^i \wedge d\overline{z^j}.$$
We now apply this construction to the Beauville-Mukai system.
When $X$ contains a smooth curve $C$ of genus $g$ by Riemann-Roch $C$ moves in a linear system $|C| \cong \bp^g$ of dimension $g$. Denote by $\mathcal{C}/\bp^g$ the universal family of all curves in the linear system $|C|$ and by $\cj$ the compatified Jacobian of degree $k$ divisors on this family. In this situation the Beauville-Mukai system is the fibration $\cj \rightarrow \bp^g$ whose generic fiber is a $g$-dimensional abelian variety which is non-canonically isomorphic with the Jacobian of the corresponding curve in the linear system. Denote by $B_{reg} \bp^g$ the regular part of the the fibration corresponding to generic fibers.
We have the following exact sequence:
$$0 \rightarrow T \cj_b \rightarrow T\cj|\cj_b \rightarrow \pi^* T_b \bp^g \rightarrow 0.$$
The normal bundle of $\Sigma$ in $X$ is isomorphic to $T^*\Sigma=K_\Sigma$ and therefore the tangent space of the moduli space $M$ at the point $b$ is $H^0(\Sigma,K_\Sigma)$. 

Curves in the linear system $|NC|$ become spectral curves in the compactified cotangent bundle $\overline{T^* C}$. In both $T^* C$ and the K3 surface $X$, the normal bundle to $\Sigma$ is $T^*\Sigma=K_\Sigma$ and therefore,
$$0 \rightarrow T \Sigma \rightarrow TX|_\Sigma \rightarrow K_\Sigma \rightarrow 0$$
gives an extension class in
$$\mathrm{Ext}^1(K_\Sigma,T \Sigma) \cong H^0(\Sigma,K_\Sigma^{\otimes 3})^\vee \rightarrow H^0(\Sigma,K_\Sigma)^{\otimes3}.$$
This class is the Donagi-Markman cubic at $b \in \bp^g$ as in \cite{donagi1997nilpotent}.

\begin{example}
Let $\pi: X \rightarrow \bp^1$ be an elliptic K3 surface written in the Weierstrass form
$$y^2=x^3+f(z)x+g(z).$$
For a given polynomial 
$$p(z)=u_0+u_1z+ \dots + u_n z^n,$$
we obtain a hyperelliptic curve $\Sigma$ defined via the equation $x=p(z)$, or equivalently
$$y^2=p(z)^3+f(z)p(z)+g(z).$$
In this situation the symplectic surface $X$ is foliated by fibers of the elliptic fibration and $\Sigma$ defines a spectral curve in the sense of KS.
\end{example}

\begin{question}
Is it true that the prepotential for this class of examples coincides with the Seiberg Witten prepotential?
\end{question}

It is reasonable to expect that an analogue of Theorem~\ref{main} exists for Beauville-Mukai systems.  It may be related to \cite{BKSAir} where Airy structures and topological recursion are considered on a class of singular spectral curves.

\begin{thm}
Let $\pi: M_H(v) \rightarrow |C|$ be the Beauville-Mukai associated with the K3 surface $X$ and a curve $C$. Then the tensor $A$ induces the Donagi-Markman cubic for the Beauville-Mukai system.
\end{thm}
\begin{proof}
I think the proof of theorem 1 should work here as well since the Rauch variational formula proved in the appendix works in this case as well.
\end{proof}

Bogomolov-Beauville quadratic form on the moduli space

\begin{question}
In the case of Hitchin systems there is a connection between the prepotential and the special K\"ahler metric. Is the same relation true here in terms of the Bogomolov-Beauville quadratic form?
\end{question}

==> bergmann.tex <==
\section{Free energy associated with Airy structures}


In this section we study the formal germ of the deformation space $\cb$ around every point $\Sigma_0$. We first define a collection of analytic functions $F^h$ for every $h \geq 1$ in a small neighbourhood $U$ of this point. Let us fix a collection of local coordinates $z^i$ of the open subset $U$, for $i=1, \dots, g$ around the point $\Sigma_0$.
For any point $\Sigma$ in the neighbourhood $U$ there is an element $\omega_{h,1}(\Sigma) \in \cG_{\Sigma}$. 
The collection of vector spaces $\cG_{\Sigma}$ give rise to an infinite dimensional vector bundle $\cG$ on the deformation space $\cb$. 
Recall that the foliation $\cF$ induces a flat connection $\nabla_{\cF}$ on the vector bundle $\cG$. 
This induces a connection on the vector bundle $\ch$ which coincides with the Gauss-Manin connection. Every point $\Sigma$ on the deformation space $\cb$ gives a Quantum Airy structure on $V_{\Sigma} \subset \cG_{\Sigma}$ consisting of meromorphic differentials with zero $A$-periods. In particular, for any such point 
the vector $\omega_{h,1}(\Sigma) \in V_{\Sigma}$ defines a vector $[\omega_{h,1}(\Sigma)] \in \ch_{\Sigma}$ via the composition $V_\Sigma \hookrightarrow \cG_{\Sigma} \rightarrow \ch_\Sigma$.
A choice of $A$ and $B$-cycles defines an isomorphism $\ch_{\Sigma}\cong\bc^{2g}$, hence an isomorphism $\ch_{\Sigma}\cong\ch_{\Sigma_0}$ for nearby $\Sigma$, known as
the Gauss-Manin connection.






==> bergmanntau.tex <==
\subsubsection{Bergman tau function}

In this section we consider the case of genus one and study the connection between free energy and Bergman tau function.
Let us consider the special case $\Sigma \subset T^*C$, where $\Sigma$ is a spectral curve inside the cotangent bundle of a smooth projective curve $C$ associated with a regular point on the base of the Hitchin system. 
Consider a point $\Sigma_0$ of the deformation space $\cb$.

Using Lemma \ref{free} we can define a function $F^1: U \rightarrow \cG$ such that $dF^1(\Sigma)=\epsilon_{\Sigma_0}(\Sigma)$ for any $\Sigma \in U$. We can use this function to define the Bergman tau function associated to the deformation space $\cb$.



We now state the main result of this section: 

\begin{theorem}
The projection of the parallel transport of the element $\epsilon(\Sigma) \in V_{\Sigma}$ to the vector space $H^{0,1}(\Sigma_0;\bc)$ using the Gauss-Manin connection is the derivative of the genus one free energy. 
\end{theorem}
\begin{proof}
The parallel transport of the element $\epsilon(\Sigma)$ to the fiber $\cG_{\Sigma_0}$ is the vector $\epsilon_{\Sigma_0}(\Sigma)$. By Lemma \ref{free} its projection to the quotient space $H^{0,1}(\Sigma_0;\bc)=H^1(\Sigma_0;\bc)/H^0(\Omega^1_{\Sigma_0};\bc)$ is equal to the vector 

$$F_1^1 \eta^1 + \dots + F_g^1 \eta^g.$$
The statement now follows from the discussions in this section. 
\end{proof}

WILL MOVE TO $T^*C$ SECTION.

Define $F_1$ following \cite{eynard_orantin} adapted to $\Sigma\subset (X,\omega,\cf)$.  In a neighbourhood $U\subset B$ of $[\Sigma]$, for any $\alpha\in R$ we can define a holomorphic function $f_\alpha:U\to\bc$ by:
$$f_\alpha(p):=-\Res_{p=\alpha} \frac{dy(p)}{\frac{\partial P}{\partial x}(p)^2\frac{\partial P}{\partial y}(p)}$$
where $dy$ is pulled back to the curve $\Sigma$ defined by $P(x,y)=0$.
It is well-defined on $U$ (where $\alpha\in R$ continues to a unique choice in nearby curves).  It is easy to check that $f_\alpha(p)$ is invariant under the change of coordinates \eqref{xyamb}.  This does not depend on a choice of $A$-cycles so it defines a function on a branched cover of $\cb$ (branched over the points in $\cb$ where $\Sigma'$ has worse than simple tangencies). %For local coordinates $(x,y)$ for $X$ such that $dx\wedge dy=\omega$ and $x=$constant defines $\cf$ locally one can constrain the ambiguity \eqref{xyamb} further by also requiring that $x-y^2=0$ defines $\Sigma$ locally.  This choice of local coordinates is unique up to $(x,y)\mapsto(\zeta^2x,\zeta y)$ for $\zeta^3=1$.  Then $f_a(p):=\Res_{p=a} \frac{dy(p)dy(p)}{dx(p)}$.

The Bergman tau function $\tau_B:U\to\bc$ is defined for any choice of $L_A\cong\bz^g\subset H^1(\Sigma;\bz)$ as follows.  For locally defined coordinates $(x,y)$ as above, define $u=x(\alpha)$ to be the critical value of $x$ in each curve in the family $U\subset\cb$.  Using the Bergman kernel defined by $L_A$ and the local involution $p\mapsto\hat{p}$ defined by the foliation, define $\tau_B$ up to a constant by its local derivatives for each $\alpha\in R$:
$$\frac{\partial}{\partial u}\ln(\tau_B)=-\Res \frac{B(p,\hat{p})}{dx(p)}.$$
This should be preserved under the change of coordinate \eqref{xyamb}.

\textcolor{red}{NOT TRUE}.  If we instead use the coordinates up to $(x,y) \mapsto (\zeta^2 x,\zeta y)$ then we still need to prove that this definition at a nearby $b'\in\cb$ defines the same $\tau_B$.  It seems to suffer from the same problem.

An explanation: the vector field $\frac{\partial}{\partial u}$ does not make sense.  We need a set of coordinates for $\cb$ to define vector fields and $\{u_\alpha\mid\alpha\in R\}$ is not a set of coordinates.  Similarly, the usual Rauch variational formulas uses canonical coordinates (critical values of $x$) whereas Baraglia-Huang prove a version using instead vector fields on $\cb$.  Their result may be adaptable to this situation.  Guess:
$$\delta\ln(\tau_B)=\sum_\alpha\Res_{p=\alpha} \delta\theta(p)\frac{B(p,\hat{p})}{dx(p)dy(p)}
$$
or in terms of $z^i$
$$
\frac{\partial}{\partial z^i}\ln(\tau_B)=\sum_\alpha \Res_{p=\alpha} \omega_i(p)\frac{B(p,\hat{p})}{dx(p)dy(p)}$$

We now recall the definition of the Bergman projective connection.
Consider two fixed vectors in $ \bz^g$ and the associated characteristic $t$. The Riemann theta function with characteristic $t$ is denoted by $\theta_t: \bc^g \rightarrow \bc$ \cite{Fay73}.
The Bergman kernel associated with an odd characteristic $t$ is defined as 
$$B(p,q)=d_p d_q \ln \left( \theta_t(u(p)-u(q))\right),$$
where $u$ is the Abel-Jacobi map.
Let $\pi_1,\pi_2: \Sigma^2 \rightarrow \Sigma$ be the natural projections.
Around any fixed point $(r,r)$ on the diagonal of $\Sigma \times \Sigma$ we can find local coordinates $(p,q)$ satisfying $p \circ \pi_1=q \circ \pi_2$.
The Bergman kernel has the form
$$B(p,q)=\left( \frac{1}{(p-q)^2}+\frac{1}{6} S_B(r) + \dots \right) dp dq,$$
The holomorphic function $S_B(r)$ is called the Bergman projective connection. 

If we define

$$B_i=\sum_\alpha \Res_{p=\alpha} \omega_i(p) \frac{B(p,\hat{p})}{dx(p) dy(p)}$$


\begin{lemma}
For any $1 \leq i,j \leq g$ we have the following relation $$\frac{\partial B_i}{\partial z^j}=\frac{\partial B_j}{\partial z^i}$$
\end{lemma}
\begin{proof}
The idea is very similar to the proof of \cite[Theorem 6.3.1]{Huang} with slight modifications. We have that
$$\frac{\partial B_i}{\partial z^j}=\sum_\alpha \frac{\partial}{\partial z^j} \Res_{p=\alpha} \left( \omega_i(p)\frac{B(p,\hat{p})}{dx_\alpha(p)dy_\alpha(p)} \right)
=\sum_\alpha \sum_\beta \Res_{p=\alpha} \Res_{q=\beta} \left( \frac{\omega_i(p) \omega_j(q)}{dx_\alpha(p)dy_\alpha(p)} \cdot \frac{B(p,q) B(\hat{p},q)}{dx_\beta(q) dy_\beta(q)} \right).$$
Consider the expansion of the expressions $B(p,q)$ and $B(\hat{p},q)$:
$$B(p,q)=(b_0(q)+ b_1(q)p + \dots) dpdq,$$
$$B(\hat{p},q)=(b_0(q)- b_1(q)p + \dots) dpdq.$$
Since we are interested in the coefficient of $\frac{dp dq}{pq}$ we have that

$$\Res_{p=\alpha} \Res_{q=\beta} \left( \frac{\omega_i(p) \omega_j(q)}{dx_\alpha(p)dy_\alpha(p)} \cdot \frac{B(p,q) B(\hat{p},q)}{dx_\beta(q) dy_\beta(q)} \right)=\Res_{p=\alpha} \Res_{q=\beta}\left(\frac{\omega_i(p) \omega_j(q)}{dx_\alpha(p) dy_\alpha(p)} \cdot \frac{b_0(q)^2}{dx_\beta(q) dy_\beta(q)} \right)$$

This implies that
$$\sum_\alpha \sum_\beta \Res_{p=\alpha} \Res_{q=\beta} \left(\frac{\omega_i(p) \omega_j(q)}{dx_\alpha(p)dy_\alpha(p)} \cdot \frac{B(p,q) B(\hat{p},q)}{dx_\beta(q) dy_\beta(q)}\right)=\sum_\alpha \sum_\beta \Res_{p=\alpha} \Res_{q=\beta} \left( \frac{\omega_i(p) \omega_j(q)}{dx_\alpha(p)dy_\alpha(p)} \cdot \frac{B(p,q) B(p,q)}{dx_\beta(q) dy_\beta(q)}\right),$$
which proves the statement since the last expression is symmetric in $i,j$.
\end{proof}

\begin{definition}
The Bergman tau-function $\tau_B$ is the solution of the equations
$$\frac{\partial \ln (\tau_B)}{\partial z^i}=B_i,$$
for all $1 \leq i \leq g$.
\end{definition}


\begin{remark}
The Bergman tau function $\tau_B$ gives a flat section $\tau_B^{24}$ of a certain line bundle equipped with the connection $d_B=d+\sum_{i=1}^m 2S_B(r_i) d \lambda_i$. This is true when the moduli space is the base of the Hitchin system. In our case we need to find a suitable projective connection: again we can take a connection $d+\sum_{i=1}^g B_i dz^i$ and a suitable power of $\tau_B$ should give a flat section of this connection or its modification.
\end{remark}



where $y$ is the coordinate for $dx$. For details see \cite[Definition 6.3.3]{Huang} or \cite[Definition 4.3]{eynard_orantin}. 

The connection between the genus one free energy and Bergman tau function:

\begin{lemma}
The formula relating the Bergman tau function and the genus one free energy.
\end{lemma}
\begin{proof}
We have that
$$w_{1,1}(p_1)=\sum_{\alpha} \Res_{p=\alpha} K(p_1,p) B(p,\hat{p}),$$
where
$$K(p_1,p)=\frac{\int_{q=p}^{\hat{p}}\omega_{0,2}(p_1,q)}{\omega_{0,1}(p) - \omega_{0,1}(\hat{p})}=\frac{\int_{q=p}^{\hat{p}}B(p_1,q)}{\omega_{0,1}(p) - \omega_{0,1}(\hat{p})}$$
Therefore
$$w_{1,1}(p_1)=\sum_{\alpha} \Res_{p=\alpha} \frac{\int_{q=p}^{\hat{p}}B(p_1,q)}{y_\alpha(p)dx_\alpha(p)-y_\alpha(\hat{p})dx_\alpha(\hat{p})} \cdot B(p,\hat{p})$$
We choose local coordinate $z_\alpha$ around the ramification point $r_\alpha$ such that $x_\alpha(p)=x_\alpha(r_\alpha)+z_\alpha(p)^2$.
Now consider the expansion of the following expressions when we are close to the ramification point $r_\alpha$:


$$y_\alpha(p)=y_\alpha(r_\alpha)+y^{'}_\alpha(r_\alpha)z_\alpha(p) + \frac{1}{2}y^{''}_\alpha(r_\alpha)z^2_\alpha(p) + \frac{1}{6}y^{'''}_\alpha(r_\alpha)z^3_\alpha(p) + \dots$$
$$\omega_{0,1}(p)-\omega_{0,1}(\hat{p})=4z_\alpha^2(p) \left(y^{'}_\alpha(r_\alpha)+\frac{1}{6}y^{'''}_\alpha(r_\alpha)z^2_\alpha(p) + \dots \right) dz_\alpha(p)$$
$$\omega_i(p)=\left(\omega_i(r_\alpha)+ \omega_i^{'}(r_\alpha) z_\alpha(p)+ \frac{1}{2} \omega_i^{''}(r_\alpha) z_\alpha(p)^2 +\dots \right) dz_\alpha(p)$$
This implies that
$$\int_{p_1 \in b_i} w_{1,1}(p_1)=\sum_{\alpha} \Res_{p=\alpha} \frac{z_\alpha(p)(\omega_i(r_\alpha)+\frac{1}{6} \omega_i^{''}(r_\alpha) z_\alpha^2(p) +\dots )}{4z_\alpha^2(p) \left(y^{'}_\alpha(r_\alpha)+\frac{1}{6}y^{'''}_\alpha(r_\alpha)z^2_\alpha(p) + \dots \right) dz_\alpha(p)} \cdot B(p,\hat{p})$$
$$=\frac{1}{4}\sum_\alpha \Res_{p=\alpha} \omega_i(p) \frac{B(p,\hat{p})}{dx(p) dy(p)}+\sum_{\alpha} \frac{1}{y^{'}_\alpha(r_\alpha)}\left( \omega_i^{''}(r_\alpha)-\frac{y^{'''}_\alpha(r_\alpha)}{y^{'}_\alpha(r_\alpha)} \cdot \omega_i(r_\alpha) \right)$$
$$=\frac{B_i}{4}+\sum_{\alpha} \frac{1}{y^{'}_\alpha(r_\alpha)}\left( \omega_i^{''}(r_\alpha)-\frac{y^{'''}_\alpha(r_\alpha)}{y^{'}_\alpha(r_\alpha)} \cdot \omega_i(r_\alpha) \right)$$

We know that the first term is the partial derivative of $\ln \tau_B$.
It might be true that the second term is also the partial derivative of a function. In the case of Hitchin systems it is the derivative of $\prod y_\alpha^{'}(r_\alpha)$.
\end{proof}


\begin{corollary}
The Bergman tau function for Hitchin system.
\end{corollary}
\begin{proof}
This follows since there is a cancellation coming from the varitational formulas for the Hitchin system.  
\end{proof}


==> local_to_global.tex <==
\section{From local to global}

In Section \ref{deformationofcurvessection} we studied a family $\mathcal{B}$ of curves $\Sigma$ embedded in a foliated symplectic surface $(S,\Omega_S,\mathcal{F})$ and the embedding of an open neighbourhood $\mathcal{B}_{\Sigma_0}$ into a fiber $\mathcal{H}_{\Sigma_0} = H^1(\Sigma_0,\mathbb{C})$. All consideration were done at the level of cohomology which gives a `global' picture of the deformation. In Section \ref{theembeddingofdiscssection} we studied what deformation of $\Sigma$ looks like near a ramification point and the embedding of $Discs^{\epsilon, M}_{t_0}$ into $W^{\epsilon, M}_{t_0}$, which is a `local' picture of the deformation. The idea of this section is to connect the two pictures together by lifting each cohomological classes in Section \ref{deformationofcurvessection} to differential forms with Laurent series expansions near ramification points given by series introduced in Section \ref{theembeddingofdiscssection}.  

Recall the set up in Section \ref{deformationofcurvesinfamilysubsection} with a family $\mathcal{B}$ of curves $\Sigma$ embedded in a foliated symplectic surface $(S,\Omega_S,\mathcal{F})$. Let us pick a reference point $[\Sigma_0] \in \mathcal{B}_{\Sigma_0}$. Fix a collection of $(\mathcal{F}, \Omega_S)$-charts $\mathcal{U}_{Ram} := \{(U_{\alpha\in Ram}, x_{\alpha \in Ram}, y_{\alpha \in Ram})\}$ such that $r_\alpha(\Sigma_0) \in U_\alpha$ where $r_\alpha(\Sigma_0), \alpha \in Ram$ are ramification points of $\Sigma_0$, $\Sigma_0\cap U_\alpha$ is bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with the standard local coordinate $z_\alpha := \sqrt{x_\alpha - x_\alpha(r_\alpha)}$. We choose $\mathcal{B}_{\Sigma_0}$ to be sufficiently small such that for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$, $\Sigma \cap U_\alpha$ contains the ramification point $r_\alpha(\Sigma)$ of $\Sigma$ and it is bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with standard local coordinate $z_\alpha := \sqrt{x_\alpha - x_\alpha(r_\alpha(\Sigma))}$. For each $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ the parameterization of $\Sigma\cap U_\alpha$ takes the form
\begin{equation*}
    t_\alpha(\Sigma) = (x_\alpha = a_\alpha(\Sigma) + z^2_\alpha,\ y_\alpha = b_{0\alpha}(\Sigma) + b_{1\alpha}(\Sigma)z_\alpha + b_{2\alpha}(\Sigma)z^2_\alpha + ...).
\end{equation*}

Let us emphasize that the coefficients $\{a_\alpha(\Sigma), b_{0\alpha}(\Sigma), b_{1\alpha}(\Sigma), b_{2\alpha}(\Sigma),...\}$ depends on our choice of the local coordinates $(x_\alpha, y_\alpha)$. In particular, we choose $(x_\alpha, y_\alpha)$ such that a reference point $[\Sigma_0] \in \mathcal{B}$ is parameterized by $t_{\alpha}(\Sigma_0) = (x_\alpha = z^2_\alpha, y_\alpha = z_\alpha)$.

Let us pick $\{\epsilon_{\alpha \in Ram} \in \mathbb{R}\}$ and $\{M_{\alpha \in Ram} \in \mathbb{R}\}$ such that $0 < \epsilon_\alpha < M_\alpha$ and define the following discs and annulus on $\Sigma$ for $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ :
\begin{align*}
    \mathbb{D}_{\alpha, \epsilon_\alpha}(\Sigma) &:= \{p \in \Sigma\cap U_\alpha\ |\ |z_\alpha(p)| < \epsilon_\alpha\} \subset \Sigma\cap U_\alpha\\
    \mathbb{D}_{\alpha, M_\alpha}(\Sigma) &:= \{p \in \Sigma\cap U_\alpha\ |\ |z_\alpha(p)| < M_\alpha\} \subset \Sigma\cap U_\alpha\\
    \mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}(\Sigma) &:= \mathbb{D}_{\alpha, M_\alpha} - \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}.
\end{align*}
We suppose that $\mathcal{B}_{\Sigma_0}$ is chosen to be sufficiently small such that $\bar{\mathbb{D}}_{\alpha,M_\alpha}(\Sigma) \subset \Sigma\cap U_\alpha \subset \Sigma$ for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$, in other words, $\mathbb{D}_{\alpha,M_\alpha}(\Sigma)$ is properly contained inside the coordinate chart $\Sigma\cap U_\alpha$ for all $[\Sigma]\in \mathcal{B}_{\Sigma_0}$. Consequently, $\sum_{k=0}^\infty b_{k\alpha}(\Sigma)z^k_\alpha$ converges in an open set containing $\mathbb{D}_{\alpha, M_\alpha}(\Sigma)$ for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ and so we have the map $\gamma_\alpha : \mathcal{B}_{\Sigma_0} \hookrightarrow Discs^{M_{\alpha}}$ given by $[\Sigma]\mapsto t_\alpha(\Sigma) \in Discs^{M_\alpha}$.

Over $Discs^{M_\alpha}$ for each $\alpha \in Ram$ we have the vector bundle $W^{\epsilon_\alpha, M_\alpha} \rightarrow Discs^{M_\alpha}(\Sigma)$ as defined in Section \ref{theembeddingofdiscssection}. Locally we treat a curve $\Sigma \subset S$ as an embedding of $|Ram|$ discs $\mathbb{D}_{\alpha, M_\alpha} \subset U_\alpha \cong \mathbb{C}^2$ indexed by the ramification index set $Ram$. Therefore, it makes sense to introduce 
\begin{equation*}
    Discs^{Ram} := \prod_{\alpha \in Ram}Discs^{M_\alpha}, \qquad Discs^{Ram}_{t} := \prod_{\alpha \in Ram}Discs^{\epsilon_\alpha, M_\alpha}_{t_{\alpha}}, \qquad W^{Ram} := \prod_{\alpha \in Ram}W^{\epsilon_\alpha, M_\alpha}.
\end{equation*}
So $W^{Ram}\rightarrow Discs^{Ram}$ is a trivial vector bundle where each fiber over $t = (t_{\alpha \in Ram}) \in Discs^{Ram}$ is $W^{Ram}_t = W^{Ram}_{Airy} := \prod_{\alpha \in Ram}W^{\epsilon_\alpha, M_\alpha}_{Airy}$. A typical element $\xi \in W^{Ram}_{t}$ can be written as $\xi = \sum_{\alpha \in Ram} [\alpha]\otimes\xi_\alpha$ where $\xi_\alpha \in W^{\epsilon_\alpha, M_\alpha}_{t_\alpha}$.
We define the symplectic form $\Omega$ and the connection $\nabla$ for $W^{Ram}$ in an obvious way: $\Omega_t := \Omega_{Airy}$ where $\Omega_{Airy}([\alpha_1]\otimes \xi_{1}, [\alpha_2]\otimes \xi_{2}) := \delta_{\alpha_1,\alpha_2}Res_{z=0}(\xi_1\int\xi_2)$ and $\nabla \xi := \sum_{\alpha\in Ram}[\alpha]\otimes \nabla_\alpha \xi_\alpha$ where $\nabla_\alpha$ is a connection for $W^{\epsilon_\alpha, M_\alpha}$ as defined in Section \ref{theembeddingofdiscssection}. It is clear that $(W^{Ram}\rightarrow Discs^{Ram}, \Omega, \nabla)$ is a weak symplectic vector bundle and $\Omega_{Airy}$ is $\nabla$-covariantly constant.  From the universal properties of direct product, the collection of maps $\gamma_\alpha : \mathcal{B}_{\Sigma_0} \hookrightarrow Discs^{M_{\alpha}}$ induces 
\begin{equation}\label{gammamapbtodiscs}
    \gamma := \prod_{\alpha\in Ram}\gamma_\alpha : \mathcal{B}_{\Sigma_0} \hookrightarrow Discs^{Ram}.
\end{equation}
In fact, if $\mathcal{B}_{\Sigma_0}$ is sufficiently small then the image of $\gamma$ will even be in $Discs^{Ram}_{t_{0}}$, where $t_0 := (t_{0\alpha\in Ram}) \in Discs^{Ram}$ and $t_{0\alpha} := t_\alpha(\Sigma_0)$. 

Using the map $\gamma$ we obtain the pull-back bundle $\gamma^*W^{Ram}\rightarrow \mathcal{B}_{\Sigma_0}$ with the connection $\gamma^*\nabla$. We define the pull-back connection $\gamma^*\nabla$ as follows. For any $\xi \in \Gamma(Discs^{Ram}, W^{Ram})$ we have $\gamma^*\xi \in \Gamma(\mathcal{B}_{\Sigma_0},\gamma^*W^{Ram})$ with $(\gamma^*\xi)_{\Sigma} := \xi_{\gamma(\Sigma)} = \xi_{t(\Sigma)} = \sum_{\alpha \in Ram}[\alpha]\otimes (\xi_{\alpha})_{t_\alpha(\Sigma)}$ and $\gamma^*\nabla$ is defined via the properties $(\gamma^*\nabla)(\gamma^*\xi) := \gamma^*(\nabla\xi)$. Writing this down explicitly, we have
\begin{align*}
    (\gamma^*\nabla)(\gamma^*\xi)_\Sigma &:= \sum_{k = 1}^g\sum_{\alpha \in Ram, l}du^k[\alpha]\otimes\left(\frac{\partial a_\alpha(\Sigma)}{\partial u^k}\frac{\partial}{\partial a_\alpha} + \frac{\partial b_{l\alpha}(\Sigma)}{\partial u^k}\frac{\partial}{\partial b_{l\alpha}} - \frac{\partial a_\alpha(\Sigma)}{\partial u^k}\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)(\xi_{\alpha})_{t_\alpha(\Sigma)}\\
    &= \sum_{k=1}^gdu^k\left(\frac{\partial}{\partial u^k} - \frac{\partial a_\alpha(\Sigma)}{\partial u^k}\sum_{\alpha \in Ram}[\alpha]\otimes\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)(\gamma^*\xi)_\Sigma.
\end{align*}

\subsection{Choosing $\{\epsilon_{\alpha\in Ram}\}, \{M_{\alpha\in Ram}\}, \mathcal{U}_{Ram}$ and $\mathcal{B}_{\Sigma_0}$}

We will now write down a precise summary of how $\{\epsilon_{\alpha\in Ram}\}, \{M_{\alpha\in Ram}\}, \mathcal{U}_{Ram} = \{(U_{\alpha\in Ram}, x_{\alpha \in Ram}, y_{\alpha \in Ram})\}$ and $\mathcal{B}_{\Sigma_0}$ can be selected. Let $[\Sigma_0] \in \mathcal{B}$ be the reference point. For each $\alpha \in Ram$, we pick $\epsilon_\alpha, M_\alpha \in \mathbb{R}, 0 < \epsilon_\alpha < M_\alpha$ and $(\mathcal{F},\Omega_S)$-charts $(U_{\alpha\in Ram}, x_{\alpha \in Ram}, y_{\alpha \in Ram})$ with $r_\alpha(\Sigma_0) \in U_\alpha$ and $\mathcal{B}_{\Sigma_0} \subset \mathcal{B}$ satisfying the following conditions:

\begin{condition}\label{howtochoosebsigma0condition}~
\begin{enumerate}
    \item $\mathcal{B}_{\Sigma_0}$ can be covered by a single coordinates chart $(\mathcal{B}_{\Sigma_0}, u^1,\cdots, u^g)$.
    \item For all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ we have $\Sigma\cap U_\alpha$ bi-holomorphic to a simply-connected subset of $\mathbb{C}$ with standard local coordinate $z_\alpha := \sqrt{x_\alpha - x_\alpha(r_\alpha(\Sigma))}$ and $\bar{\mathbb{D}}_{\alpha, M_\alpha}(\Sigma) \subset \Sigma\cap U_\alpha$.
    \item For all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ the parallel transport on the vector bundle $G\rightarrow \mathcal{B}_{\Sigma_0}$ (see Definition \ref{gdefinition}) from the fiber $G_{\Sigma_0}$ to the fiber $G_{\Sigma}$ is possible according to Lemma \ref{paralleltransportinglemma} for any holomorphic differential form $\xi \in \Gamma(\Sigma, \Omega^1_{\Sigma}) \subset G_{\Sigma}$. Additionally, the image of $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}(\Sigma) \subset \Sigma$ via the map $s_{\Sigma}$  (see Definition \ref{ssigmadefinition}) is contained in $\Sigma_0\cap U_\alpha$.
    \item For all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ the parallel transport on the vector bundle $G\rightarrow \mathcal{B}_{\Sigma_0}$ from the fiber $G_{\Sigma}$ to the fiber $G_{\Sigma_0}$ is possible according to Lemma \ref{paralleltransportinglemma} for any $\xi \in G_\Sigma$ holomorphic on $\cup_{p \in \sigma_0} \Sigma \cap U_{0,p}$. Additionally, the image of $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}(\Sigma_0) \subset \Sigma_0$ via the map $s_{\Sigma_0}$ is contained in $\Sigma\cap U_\alpha$.
\end{enumerate}
\end{condition}
\begin{remark}
Another way to state the condition 2 is that there exists an open cover $\mathcal{U}_0 := \{U_{0,p\in \sigma_0}\}$ of $\Sigma_0\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}(\Sigma_0)$ such that $\Sigma_0\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}(\Sigma_0) \subset \cup_{p\in\sigma}\Sigma\cap U_p \subset \Sigma_0\setminus \cup_{\alpha \in Ram}\{r_\alpha\}$ and satisfying all conditions of Lemma \ref{sstaroperatorlemma}.
\end{remark}
Our results will be independent of the specific choices of $\{\epsilon_{\alpha\in Ram}\}, \{M_{\alpha\in Ram}\}, \mathcal{U}_{Ram}$ and $\mathcal{B}_{\Sigma_0}$ as long as they satisfy this condition. Condition \ref{howtochoosebsigma0condition} is a sufficient but not necessary condition for the results of this section to hold.

\subsection{The vector bundle $G\rightarrow \mathcal{B}_{\Sigma_0}$ and its properties}
\begin{definition}\label{gdefinition}
Let $G \rightarrow \mathcal{B}_{\Sigma_0}$ be a vector bundle with fiber over $[\Sigma] \in \mathcal{B}$ given by 
\begin{equation*}
    G_{\Sigma} := \left\{\xi \in \varinjlim_{\bar{\epsilon}_\alpha < \epsilon_\alpha}\Gamma(\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}, \Omega^1_\Sigma)\ |\ \oint_{\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}}\xi = 0\right\}. 
\end{equation*}
We define the connection on $G$ to be $\nabla_{\mathcal{F}} : \Gamma(\mathcal{B}_{\Sigma_0}, G)\rightarrow \Gamma(\mathcal{B}_{\Sigma_0}, T^*\mathcal{B}\otimes G)$, a differentiation along the leaf of the foliation $\mathcal{F}$.
\end{definition}
% $\Gamma(\mathcal{B}_{\Sigma_0}, G)$ is a set of global smooth section of $G$ = differential forms smooth w.r.t. \{u_i\} on (\Sigma - discs) = any differential form that look like f(x,u)dx on (\Sigma - discs) that is smooth in u. 
\begin{definition}
For any $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ we define 
\begin{equation*}
    V_\Sigma := \left\{\xi \in G_\Sigma\ |\ \oint_{A_i} \xi = 0, \forall i = 1,...,g\right\} \subset G_\Sigma.
\end{equation*}
\end{definition}
%We need to explain that this is related to $\mathcal{V}_{\Sigma} \subset H^1(\Sigma, \mathbb{C})$ and what happened if we choose different normalization for Bergman kernel.
What we meant is that if $\xi \in G_\Sigma$ then $\xi$ is a holomorphic differential on some open neighbourhood of $\Sigma\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}$. In particular, it is holomorphic on some open set containing $\bar{\mathbb{A}}_{\alpha, \epsilon_\alpha, M_\alpha}$. The Laurent series representation of $\xi$ in the standard local coordinates center at $z_\alpha = 0$ for each $\alpha \in Ram$ converges absolutely for $\bar{\epsilon}_\alpha < |z| < \bar{M}_\alpha$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha < M_\alpha < \bar{M}_\alpha$ and contains no $\frac{dz}{z}$ term because $\oint_{\partial \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}}\xi = 0$. This therefore define the map $i_\alpha : G_\Sigma \hookrightarrow W^{\epsilon_\alpha, M_\alpha}_{t_\alpha(\Sigma)}$. Performing the Laurent expansion at every ramification points of $\Sigma$ we obtain the map
\begin{equation*}
    i := \prod_{\alpha \in Ram}i_\alpha : G_\Sigma \hookrightarrow W^{Ram}_{t(\Sigma)}
\end{equation*}
for any $\Sigma \in \mathcal{B}_{\Sigma_0}$.
In this sense, we can think of $G\rightarrow \mathcal{B}_{\Sigma_0}$ as a subbundle of $W^{Ram}\rightarrow Discs^{Ram}_{t_0}$. We can apply the symplectic form $\Omega_{Airy}$ on vectors in $G_{\Sigma}$. In fact, using Riemann-bilinear identity we can obtain a nice alternative expression. For $\xi_1, \xi_2 \in G_\Sigma$ we have
\begin{align*}\label{omegaairyong}
    \Omega_{Airy}(i(\xi_1), i(\xi_2)) &= \sum_{\alpha \in Ram}Res_{z_\alpha =0}\left(i_\alpha(\xi_1)\int i_\alpha(\xi_2)\right) = \frac{1}{2\pi i}\sum_{\alpha \in Ram}\oint_{\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}}\left(\xi_1\int \xi_2\right)\\
    &= \frac{1}{2\pi i} \sum_{k=1}^g\left(\oint_{A_k}\xi_2\oint_{B_k}\xi_1 - \oint_{B_k}\xi_2\oint_{A_k}\xi_1\right).\numberthis
\end{align*}

\begin{definition}\label{endifferentialdefinition}
Let $B(p,q)$ be the normalized Bergman kernel on $\Sigma$.
For any $k \in \mathbb{Z}_{\geq 1}$ and $\alpha \in Ram$ we define 
\begin{equation*}
    \bar{e}^{k,\alpha}(p) := \frac{1}{2\pi ik}\oint_{z_\alpha = 0}\frac{B(p,q(z_\alpha))}{z_\alpha^k} \in \Gamma\left(\Sigma \setminus \cup_{\alpha \in Ram}r_\alpha,\Omega^1_{\Sigma}\right) \subset G_\Sigma.
\end{equation*}
\end{definition}
The following properties is easy to verified:
\begin{lemma}
\begin{equation*}
\oint_{p \in A_i}\bar{e}^{k,\alpha}(p) = 0 \qquad \text{and} \qquad i(\bar{e}^{k,\alpha}) = [\alpha]\otimes z^{-k}_\alpha\frac{dz_\alpha}{z_\alpha} + \sum_{k' \geq 1, \alpha' \in Ram}[\alpha']\otimes \frac{1}{k}P^{(k,\alpha),(k',\alpha')}z_{\alpha'}^{k'}\frac{dz_{\alpha'}}{z_{\alpha'}} \in W^{Ram}_{t(\Sigma)}.
\end{equation*}
\end{lemma}

Let us prove in the following that $G$ is a coisotropic subbundle of $W^{Ram}$. Recall the definition of $L^M_{Airy} \subset W^{\epsilon, M}_{Airy}$ from Section \ref{analyticresconstraintssubsection} and define $L^{Ram}_{Airy} := \prod_{\alpha \in Ram}L^{M_\alpha}_{Airy} \subset W^{Ram}_{Airy}$. We note that $T_0L^{Ram}_{Airy} = \prod_{\alpha \in Ram}T_0L^{M_\alpha}_{Airy}$, or more explicitly:
\begin{equation*}
    T_0L^{Ram}_{Airy} = \left\{\xi = \sum_{\alpha \in Ram}[\alpha]\otimes \xi_\alpha\ |\ \xi_\alpha(z) \in z\mathbb{C}[[z]]\frac{dz}{z}, \begin{array}{c}
    \text{$\xi_\alpha(z)$ converges for $|z| < \bar{M}_\alpha$}\\ 
    \text{for some $\bar{M}_\alpha > M_\alpha$}\end{array}\right\} \subset W^{Ram}_{Airy}.
\end{equation*}
\begin{lemma}\label{visgplusllemma}
For any $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ we have
\begin{equation*}
     W^{Ram}_{t(\Sigma)} = W^{Ram}_{Airy} = V_\Sigma \oplus T_0L^{Ram}_{Airy}.
\end{equation*}
Additionally, if $\xi \in V_\Sigma$ and the principal part of $i_\alpha(\xi)$ is $\sum_{k=1}^\infty \xi_{\alpha, k}z^{-k}_\alpha \frac{dz_\alpha}{z_\alpha}$ then it can be written as $\xi = \sum_{\alpha\in Ram}\sum_{k=1}^\infty \xi_{\alpha, k}\bar{e}^{k,\alpha}$.
\end{lemma}
\begin{proof}
If $\xi \in V_\Sigma$ is such that $i_\alpha(\xi)$ has no principal part for all $\alpha \in Ram$ then it must be holomorphic on $\Sigma$ and $\oint_{A_i}\eta = 0$ therefore implies that $\eta = 0$. This shows that $V_\Sigma \cap T_0L^{Ram}_{Airy} = \{0\}$.
To show that $V_\Sigma + T_0L^{Ram}_{Airy} = W^{Ram}_{Airy}$ we consider any given $\xi = (\xi_{\alpha\in Ram}) \in W^{Ram}_{Airy}$ where $\xi_\alpha \in z_\alpha^{-1}\mathbb{C}[[z_\alpha^{-1}]]\frac{dz_\alpha}{z_\alpha}\oplus z_\alpha\mathbb{C}[[z_\alpha]]\frac{dz_\alpha}{z_\alpha}$ converges absolutely for $\bar{\epsilon}_\alpha < |z_\alpha| < \bar{M}_\alpha$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha < M_\alpha < \bar{M}_\alpha$. Let $\xi_{\alpha,P} = \sum_{k=1}^\infty z^{-k}_\alpha\xi_{\alpha,k}\frac{dz_\alpha}{z_\alpha}$ be the principal part of $\xi_\alpha$. We observe that
\begin{equation}
    \sum_{k=1}^\infty \frac{\xi_{\alpha, k}}{kz^{k}_\alpha} = -\sum_{k=1}^\infty\int z^{-k}_\alpha\xi_{\alpha,k}\frac{dz_\alpha}{z_\alpha}
\end{equation}
also converges absolutely uniformly for $\bar{\epsilon}_\alpha < |z_\alpha| < \bar{M}_{\alpha}$ because integration doesn't change the radius of convergence.  Then by using the Bergman kernel $B(p,q)$ on $\Sigma$ we define
\begin{align*}
    \bar{\xi}_{\alpha}(p) := \frac{1}{2\pi i}\oint_{z_\alpha \in \partial \bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}}\left(\sum_{k=1}^\infty \frac{\xi_{\alpha, k}}{kz^{k}_\alpha}\right)B(p,q(z_\alpha))
    = \sum_{k=1}^\infty\frac{\xi_{\alpha,k}}{2\pi i k}\oint_{z_\alpha = 0}\frac{B(p,q(z_\alpha))}{z_\alpha^k} = \sum_{k = 1}^\infty\xi_{\alpha,k}\bar{e}^{k,\alpha}(p),
\end{align*}
where the term-by-term integration is allowed due to the absolute uniform convergence. Therefore, $\bar{\xi} := \sum_{\alpha \in Ram}\bar{\xi}_{\alpha}$ is holomorphic for all $p \in \Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha} \supset \Sigma \setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}$ but diverges as $p$ approaches the integration path $\partial \bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}$. The principal part of $\bar{e}^{k,\alpha}$ is $z^{-k}_\alpha\frac{dz_\alpha}{z_\alpha}$ so the principal part of $i_\alpha(\bar{\xi})$ is $\xi_{\alpha,P}$ and therefore $\oint_{\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}} \bar{\xi} = 0$. We can also check that $\oint_{p\in A_i}\bar{\xi}(p) = \sum_{k=1}^\infty \xi_{\alpha, k}\oint_{p\in A_i}\bar{e}^{k,\alpha}(p) = 0$. This implies that $\bar{\xi} \in V_\Sigma$. On the other hand, because $\Sigma \in \mathcal{B}_{\Sigma_0}$ we have that $i_\alpha(\bar{\xi})$ converges absolutely for $\bar{\epsilon}_\alpha < |z| < \bar{\bar{M}}_\alpha$ where $\bar{\bar{M}}_\alpha$ is such that $\mathbb{D}_{\alpha, M_\alpha} \subset \mathbb{D}_{\alpha, \bar{\bar{M}}_\alpha} \subset \Sigma\cap U_\alpha$. It follows that $\xi_\alpha - i_\alpha(\bar{\xi})$ has zero principal part and converges absolutely for  $|z_\alpha| < \min(\bar{M}_\alpha, \bar{\bar{M}}_\alpha)$. Therefore $\xi - i(\bar{\xi}) \in T_0L^{Ram}_{Airy}$ this proves that $W^{Ram}_{Airy} = V_{\Sigma}\oplus T_0L^{Ram}_{Airy}$. In addition, if $\xi \in V_\Sigma$, then $\xi - \bar{\xi}$ is holomorphic on $\Sigma$ with $\oint_{A_i}(\xi - \bar{\xi}) = 0$ for all $i = 1,...,g$ which means $\xi = \bar{\xi} = \sum_{\alpha \in Ram}\sum_{k=1}^\infty \xi_{\alpha, k}\bar{e}^{k,\alpha}$.
\end{proof}

\begin{corollary}
For any $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ we have
\begin{equation*}
    G_{\Sigma} + T_0L^{Ram}_{Airy} = W^{Ram}_{Airy}.
\end{equation*}
\end{corollary}
\begin{proof}
This follows from Lemma \ref{visgplusllemma} and the fact that $V_\Sigma \subset G_\Sigma$.
\end{proof}

\begin{corollary}\label{vislagrangiancomplementcorollary}
$V_\Sigma$ is a Lagrangian complement of $T_0L^{Ram}_{Airy}$ in $W^{Ram}_{Airy}$. 
\end{corollary}
\begin{proof}
We already know from Lemma \ref{visgplusllemma} that $V_\Sigma$ is a complement of $T_0L^{Ram}_{Airy}$.
Using (\ref{omegaairyong}), it is clear that for any $\xi_1, \xi_2 \in V_{\Sigma}$ we would have $\Omega_{Airy}(\xi_1,\xi_2) = 0$ because $\oint_{A_i}\xi_j = 0, i = 1,...,g, j = 1,2$. If there exists $\xi_2 \in W^{Ram}_{Airy}$ such that $\Omega_{Airy}(\xi_1, \xi_2) = 0$ for all $\xi_1 \in V_{\Sigma}$ then by Lemma \ref{visgplusllemma} be write $\xi_2 = v + l$ where $v \in V_\Sigma, l \in T_0L^{Ram}_{Airy}$. But then $0 = \Omega_{Airy}(\xi_1, \xi_2) = \Omega_{Airy}(\xi_1, v+l) = \Omega_{Airy}(\xi_1,l) = 0, \forall \xi_1 \in V_{\Sigma}$ because $\Omega_{Airy}(\xi_1, v) = 0$. This can only be true if $l = 0$ because $\Omega_{Airy}$ is non-degenerates. So we have that $V_\Sigma$ is a Lagrangian subspace of $W^{Ram}_{Airy}$ i.e. $V^\perp_\Sigma = V_\Sigma$. 
\end{proof} 

\begin{lemma}\label{gperplemma}
The vector bundle $G \rightarrow \mathcal{B}_{\Sigma_0}$ is a coisotropic vector subbundle of $W^{Ram}\rightarrow Discs^{Ram}$ with the perpendicular vector bundle $G^\perp \rightarrow \mathcal{B}_{\Sigma_0}$ where each fiber is given by 
\begin{equation*}
    G^\perp_{\Sigma} := \varinjlim_{\bar{\epsilon}_\alpha < \epsilon_\alpha}d\Gamma(\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}, \mathcal{O}_{\Sigma}) \subset G_\Sigma
\end{equation*}
for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$.
\end{lemma}
\begin{proof}
From $V_\Sigma \subset G_\Sigma$ and Corollary \ref{vislagrangiancomplementcorollary} we have that $G^\perp_{\Sigma} \subset V^\perp_\Sigma = V_\Sigma \subset G_\Sigma$. 
Let us find $G^\perp_{\Sigma}$. If $\xi \in G^\perp_\Sigma$ then $\xi \in G_\Sigma$ which means $\oint_{\partial \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}}\xi = 0$. Using (\ref{omegaairyong}) we can see that the only way $\Omega_{Airy}(\xi, \eta) = 0, \forall \eta \in G_\Sigma$ can be possible is if $\oint_{A_i}\xi = 0, \oint_{B_i}\xi = 0, i = 1,...,g$. We can now define $f(p) := \int_{p_0}^p\xi$ which is a holomorphic function in an open neighbourhood of $\Sigma \setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}$.
\end{proof}

\begin{proposition}
The sympectic reduction of $W^{Ram}$ is given by $W^{Ram}//G^\perp := G/G^\perp \cong \mathcal{H}$. For any $[\Sigma]\in \mathcal{B}_{\Sigma_0}$ we have $G_\Sigma/G^\perp_\Sigma \cong \mathcal{H}_\Sigma = H^1(\Sigma, \mathbb{C})$ is a symplectic vector space with the induced symplectic form
\begin{equation}
    \tilde{\Omega}_{Airy}([\xi_1],[\xi_2]) := \Omega_{Airy}(\xi_1, \xi_2).
\end{equation}
The induced symplectic form $\tilde{\Omega}_{Airy}$ coincides with the symplectic form $\Omega_{\mathcal{H}}$ on $\mathcal{H}\rightarrow \mathcal{B}$ as introduced in Section \ref{deformationofcurvessection}.
\end{proposition}
\begin{proof}
First, we will show that $G_\Sigma/G^\perp_\Sigma$ is indeed isomorphic to the deRham cohomology group $\mathcal{H}_\Sigma = H^1(\Sigma, \mathbb{C})$.
For any set $\{\bar{\epsilon}_{\alpha\in Ram}\}$ such that $\bar{\epsilon}_\alpha < \epsilon_\alpha, \alpha\in Ram$ we have the presentation 
\begin{equation*}
    \mathcal{H}_\Sigma = H^1(\Sigma,\mathbb{C}) \cong \frac{\left\{\xi \in \Gamma\left(\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha},\Omega^1_\Sigma\right)\ |\ \oint_{\partial \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}}\xi = 0\right\}}{d\Gamma(\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}, \mathcal{O}_{\Sigma})}.
\end{equation*}
To obtain this, we may use Mayer–Vietoris sequence to get $H^1(\Sigma, \mathbb{C}) \cong \{\xi \in H^1(\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}, \mathbb{C})\ |\ \oint_{\partial \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}}\xi = 0\}$. Then by the Analytic de Rham Theorem
\cite{zein2013sheaf} and the fact that non-compact Riemann surface such as $\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}$ is a Stein manifold we have $H^1(\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}, \mathbb{C}) \cong H^1(\Gamma(\Sigma \setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}, \Omega^1_\Sigma))$ and we get the claimed presentation. Applying the fact that taking direct limit preserves short exact sequences to the above presentation for $H^1(\Sigma, \mathbb{C})$ and compare the result to the explicit expression of $G_\Sigma$ and $G^\perp_\Sigma$ in Definition \ref{gdefinition} and Lemma \ref{gperplemma}, we have $H^1(\Sigma, \mathbb{C}) = \varinjlim_{\bar{\epsilon}_\alpha < \epsilon_\alpha} H^1(\Sigma, \mathbb{C}) \cong G_\Sigma/G^\perp_\Sigma$.

Next, we show that $\tilde{\Omega}_{Airy}$ is a symplectic form on $\mathcal{H}_\Sigma$. If $\xi_1' = \xi_1 + df_1, \xi_2' = \xi_2 + df_2$ then $\tilde{\Omega}_{Airy}([\xi'_1], [\xi'_2]) = \Omega_{Airy}(\xi_1 + df_1, \xi_2 + df_2) = \Omega_{Airy}(\xi_1, \xi_2) = \tilde{\Omega}_{Airy}([\xi_1],[\xi_2])$, so $\tilde{\Omega}_{Airy}$ is well-defined. It is non-degenerates because if $[\xi] \in \mathcal{H}_\Sigma$ is such that $\tilde{\Omega}_{Airy}([\xi], [\eta]) = 0$ for all $[\eta] \in \mathcal{H}_\Sigma$ then $\Omega_{Airy}(\xi, \eta) = 0$ for all $\eta \in G_{\Sigma}$ implying that $\xi \in G^\perp_\Sigma$ and hence $[\xi] = 0$. This proves that $\mathcal{H}_\Sigma$ is a symplectic vector space with the induced symplectic form $\tilde{\Omega}_{Airy}$. Using (\ref{omegaairyong}) we can see that $\tilde{\Omega}_{Airy}$ coincides with $\Omega_{\mathcal{H}}$ as claimed.
\end{proof}

\subsection{Connection $\nabla_{\mathcal{F}}$ and parallel transports on $G\rightarrow \mathcal{B}_{\Sigma_0}$}
Let us discuss the connection $\nabla_{\mathcal{F}}$ of $G$ more explicitly. Consider $[\Sigma] \in \mathcal{B}_{\Sigma_0}$. Let $\mathcal{U} := \{(U_{p\in\sigma}, x_{p\in\sigma}, y_{p\in\sigma}\}$ be a collection of $(\mathcal{F}, \Omega_S)$-charts covering $\Sigma\setminus \cup_{\alpha\in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}(\Sigma)$ where $\Sigma\cap U_p$ are bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with $x_p$ as a local coordinate. It follows that $dx_p|_{\Sigma \cap U_p}\neq 0$ and so $r_\alpha(\Sigma) \notin \Sigma \cap U_p$ for all $\alpha \in Ram$.

Let $\{u^1,...,u^g\}$ be the local coordinates of $\mathcal{B}$ defined on $\mathcal{B}_{\Sigma_0}$.
Given a section $\xi \in \Gamma(\mathcal{B}_{\Sigma_0}, G)$, $\xi_\Sigma \in G_\Sigma$ and a tangent vector $v = \sum_{k=1}^gv^k\frac{\partial}{\partial u^k} \in T_{[\Sigma]}\mathcal{B}_{\Sigma_0}$ then for each $p \in \sigma$ we have $\iota_{v}\nabla_{\mathcal{F}}\xi|_{\Sigma \cap U_{p}} = \sum_{k=1}^gv^k\frac{\partial}{\partial u_k}|_{x_p = const}(\xi|_{\Sigma \cap U_p})$. Using $x_p$ as a local coordinates on $\Sigma \cap U_p$ and write $\xi|_{\Sigma\cap U_p} = \xi_p(x_p,u)dx$. It follows that $\iota_v\nabla_{\mathcal{F}}\xi|_{\Sigma \cap U_{p}} = \sum_{k=1}^g v^k\frac{\partial}{\partial u^k}(\xi_p(x_p,u))dx_p$. We patch $\iota_v\nabla_{\mathcal{F}}\xi|_{\Sigma\cap U_p}$ for each $p \in\sigma$ together to obtain $\iota_v\nabla_{\mathcal{F}}\xi$ which is holomorphic on $\Sigma \setminus \bar{\mathbb{D}}_{\alpha, \bar{\epsilon}}(\Sigma)\subset \cup_{p\in \sigma}\Sigma \cap U_p$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha, \forall \alpha \in Ram$. Let us show that $\oint_{\partial \bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}(\Sigma)}\nabla_{\mathcal{F}}\xi = 0$. Write $\xi$ on $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}(\Sigma)$ in the standard local coordinates as $\xi(z_\alpha) = \sum_{k\neq 0} \xi_{\alpha,k}z^k_\alpha \frac{dz_\alpha}{z_\alpha}$. Since $x_\alpha = a_\alpha(\Sigma) + z^2_\alpha$, we have $\nabla_{\mathcal{F}}(z_\alpha) = \sum_{k=1}^gdu^k\frac{\partial a_\alpha(\Sigma)}{\partial u^k}\frac{\partial}{\partial a_\alpha}|_{x_\alpha = const}z_\alpha = -\frac{1}{2z_\alpha}\sum_{k=1}^gdu^k\frac{\partial a_\alpha(\Sigma)}{\partial u^k}$. It follows that $\nabla_{\mathcal{F}}(z_\alpha^kdz_\alpha) = \frac{1}{2}\sum_{k=1}^gdu^k\frac{\partial a_\alpha(\Sigma)}{\partial u^k}(1-k)z^{k-2}_\alpha dz_\alpha$, therefore $\iota_v\nabla_{\mathcal{F}}\xi$ is free of $\frac{dz_\alpha}{z_\alpha}$ term. Hence $\iota_v\nabla_{\mathcal{F}}\xi \in G_{\Sigma}$, in other words,  $\nabla_{\mathcal{F}}\xi \in \Gamma(\mathcal{B}_{\Sigma_0},T^*\mathcal{B}\otimes G)$.

\begin{lemma}
The vector bundle $G\rightarrow \mathcal{B}_{\Sigma_0}$ with the connection $\nabla_{\mathcal{F}}$ is flat.
\end{lemma}
\begin{proof}
The Lemma follows because on each $\Sigma \cap U_p$ we have 
\begin{equation*}
d_{\nabla_{\mathcal{F}}} \xi|_{\Sigma\cap U_p} = \nabla_{\mathcal{F}}\xi_{\Sigma\cap U_p} = \sum_{k=1}^gdu^k\frac{\partial}{\partial u^k}(\xi_p(x_p,u)dx_p)    
\end{equation*}
 and
 \begin{equation*}
     d^2_{\nabla_{\mathcal{F}}} \xi|_{\Sigma\cap U_p} = \sum_{k=1}^gdu^k\wedge \nabla_{\mathcal{F}}\frac{\partial}{\partial u^k}(\xi_p(x_p,u)dx_p) = \sum_{k,l = 1}^gdu^k\wedge du^l\frac{\partial^2}{\partial u^k\partial u^l}(\xi_p(x_p,u)dx_p) = 0.
 \end{equation*}
 Therefore, $d^2_{\nabla_{\mathcal{F}}} = 0$ and so $\nabla_{\mathcal{F}}$ is flat.
\end{proof}

Let us turn our attention to parallel transports on $G$ using the connection $\nabla_{\mathcal{F}}$. Since the connection is flat, the parallel transport will be path-independent. As we will see, the parallel transport of $\xi \in G_{\Sigma}$ to the fiber $G_{\Sigma'}$ only exists if $[\Sigma] \in \mathcal{B}$ is close enough to $[\Sigma'] \in \mathcal{B}$.

We suppose that for any $(\mathcal{F}, \Omega_S)$-chart $(U_p,x_p,y_p) \in \mathcal{U}$, if $p' \in U_p$ then $p'$ is path-connected to  $\Sigma\cap U_p$ via a leaf of the foliation $x_p = const$. Let $[\Sigma'] \in \mathcal{B}_{\Sigma_0}$ be sufficiently close to $[\Sigma]$ such that $\Sigma' \setminus \cup_{\alpha\in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}(\Sigma') \subset \cup_{p \in \sigma}U_p$ and $\Sigma'\cap U_p$ is bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with $x_p$ as a local coordinate. In other words, $dx_p|_{\Sigma' \cap U_p}\neq 0$ and so $r_\alpha(\Sigma') \notin \Sigma' \cap U_p$ for all $\alpha \in Ram$.

\begin{definition}\label{ssigmadefinition}
We define the map $s_{\Sigma'}:\cup_{p \in \sigma}\Sigma'\cap U_p\rightarrow \cup_{p \in \sigma}\Sigma\cap U_p$ by sending any point $q' \in \cup_{p \in \sigma}\Sigma'\cap U_p$ to $q \in \cup_{p \in \sigma}\Sigma\cap U_p$ along a leaf of foliation.
\end{definition}
By our choice of the covering $\mathcal{U}$ and the properties of foliation, $s_{\Sigma'}$ is indeed well-defined and one-to-one. We claim that any differential form $\xi \in G_{\Sigma}$ defined on $\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}(\Sigma)$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha$ such that $\cup_{p\in \sigma}\Sigma\cap U_p\subset \Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}(\Sigma)$, then its pull-back $s_{\Sigma'}^*\xi$ is in $G_{\Sigma'}$. Let us verify that this is indeed the case. Since $\cup_{p\in \sigma}U_p$ contains ramification points of neither $\Sigma$ nor $\Sigma'$ therefore $x_p$ will be a local coordinates for both $\Sigma\cap U_p$ and $\Sigma'\cap U_p$. In $x_p$ local coordinates, we can express $s_{\Sigma'}$ as
\begin{equation*}
x_p \circ s_{\Sigma'}|_{\Sigma'\cap U_p} \circ x_p^{-1} = id_{\mathbb{C}}|_{x_p(\Sigma'\cap U_p)}: x_p(\Sigma'\cap U_p)\rightarrow x_p(\Sigma'\cap U_p)\subset x_p(\Sigma\cap U_p) \subset \mathbb{C}.
\end{equation*}
In particular, $s_{\Sigma'}$ is biholomorphic to its image. It follows that $s^*_{\Sigma'}\xi|_{\Sigma'\cap U_p}$ is holomorphic for all $p \in \sigma$. But $\Sigma'\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}(\Sigma') \subset \cup_{p\in \sigma}\Sigma'\cap U_p$, so there exists $\bar{\epsilon}'_\alpha < \epsilon_\alpha, \forall\alpha \in Ram$ such that $\Sigma'\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma')\subset \Sigma'\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}'_\alpha}(\Sigma') \subset \cup_{p\in \sigma}\Sigma'\cap U_p$ and therefore $s^*_{\Sigma'}\xi \in \varinjlim_{\bar{\epsilon}'_\alpha < \epsilon_\alpha}\Gamma(\Sigma'\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}'_\alpha}(\Sigma'), \Omega^1_{\Sigma'})$. Lastly, given $\oint_{\partial\bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma)}\xi = 0$ we need to check that $\oint_{\partial\bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}(\Sigma')}s^*_{\Sigma'}\xi = 0$, but this follows from the Lemma below:
\begin{lemma}\label{integralofparalleltransportlemma}
Let $s_{\Sigma'}:\cup_{p\in\sigma}\Sigma'\cap U_p\rightarrow \cup_{p\in\sigma}\Sigma\cap U_p$ be as given above. Then for any $\xi \in G_{\Sigma}$ holomorphic on $\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}(\Sigma) \subset \cup_{p\in\sigma}U_p$ and a path $C$ on $\Sigma'\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma')$, we have
\begin{equation*}
    \int_{C}s^*_{\Sigma'}\xi = \int_{(s_{\Sigma'})_*C}\xi.
\end{equation*}
Where $(s_{\Sigma'})_*C$ is the image of $C$ in $\Sigma\setminus \cup_{\alpha\in Ram}\bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma)$ under the map $s_{\Sigma'}$.
\end{lemma}
\begin{proof}
We dissect $C$ into closed segments $C_i, i = 1,...,N_C$ such that $C_i \subset \Sigma'\cap U_{p_i}$ for some $p_i \in \sigma$. As we have seen, $s_{\Sigma'}|_{\Sigma'\cap U_{p_i}}$ is a restriction of the identity so the Lemma holds for each segment $C_i$. Summing the integral over all segments $C_i$ proving the Lemma.
\end{proof}

Since $(s_{\Sigma'})_*(\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma'))$ is just $\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma)$, we have $\oint_{\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma')}s^*_{\Sigma'}\xi = \oint_{\partial \bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}(\Sigma)}\xi = 0$ because $\xi \in G_\Sigma$. This shows that $s^*_{\Sigma'}\xi \in G_{\Sigma'}$ as claimed.

It is important to understand that given any two points $[\Sigma], [\Sigma'] \in \mathcal{B}_{\Sigma_0}$ and any $\xi\in G_{\Sigma}$, it is not guaranteed that the pull-back $s^*_{\Sigma'}\xi$ is a well-defined vector in $G_{\Sigma'}$. This is much like the situation in Section \ref{theembeddingofdiscssection} where given $\xi\in W^{\epsilon, M}_{Airy}$ then $\exp(a\mathcal{L}_{\frac{1}{2z}\partial_z})\xi \in W^{\epsilon, M}_{Airy}$ only if $|a|$ is sufficiently small. In summary, we have the following statement analogous to Lemma \ref{expoperatorlemma}.
% This Lemma only gives a sufficient condition. It is useful theoretically for showing the existence of parallel transport in G in general. In practice we should provide an easier way, e.g. directly comparing size of a(\Sigma) - a(\Sigma_0) to \epsilon. 
\begin{lemma}\label{sstaroperatorlemma}
Let $[\Sigma], [\Sigma'] \in \mathcal{B}_{\Sigma_0}$. Given $\xi \in G_{\Sigma}$ where $\xi$ is holomorphic on $\Sigma\setminus \cup_{\alpha\in Ram}\bar{\mathbb{D}}_{\alpha,\bar{\epsilon}_\alpha}(\Sigma)$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha$. If we can cover $\Sigma\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}(\Sigma)$ with $(\mathcal{F},\Omega_S)$-charts $\mathcal{U} = \{(U_{p\in \sigma}, x_{p\in\sigma}, y_{p\in\sigma})\}$ such that $\Sigma\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}(\Sigma) \subset \cup_{p\in\sigma}\Sigma\cap U_p \subset \Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}(\Sigma)$ and satisfying the following properties:
\begin{enumerate}
    \item For each $p \in \sigma, \Sigma\cap U_p$ is bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with $x_p$ as a local coordinate.
    \item For each $p \in \sigma$, $U_p \subset S$ if $p' \in U_p$ then $p'$ is path-connected to  $\Sigma\cap U_p$ via a leaf of the foliation $x_p = const$.
    \item For each $p \in \sigma$, $\Sigma'\cap U_p$ is bi-holomorphic to a simply-connected open subset of $\mathbb{C}$ with $x_p$ as a local coordinate and $\Sigma'\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha,\epsilon_\alpha}(\Sigma') \subset \cup_{p\in\sigma}U_p$.
\end{enumerate}
Then $s^*_{\Sigma'}\xi \in G_{\Sigma'}$.
\end{lemma}

We claim that the pull-back via $s_{\Sigma'}$ is the parallel transport on $G$. The following is analogous to Lemma \ref{paralleltransportinwlemma}.
\begin{lemma}\label{paralleltransportinglemma}
Given $[\Sigma]\in \mathcal{B}_{\Sigma_0}$, $\xi\in G_{\Sigma}$ then for all $[\Sigma'] \in \mathcal{B}_{\Sigma_0}$ such that the condition of Lemma \ref{sstaroperatorlemma} is satisfied then $\xi_{\Sigma'} := s^*_{\Sigma'}\xi$ is a parallel vector field. In other words, $\xi_{\Sigma'}$ is the parallel transport of $\xi \in G_{\Sigma}$ from $[\Sigma]$ to $[\Sigma']$.
\end{lemma}
\begin{proof}
Since $x_p$ is a local coordinate of $\Sigma$ on $\Sigma \cap U_p$ we can write $\xi|_{\Sigma\cap U_p} = f(x_p)dx_p$ for some holomorphic function $f$ which is constant with respect to the coordinates of $\mathcal{B}$. Because $s^*_{\Sigma'}x_p = x_p$ by definition, we have $s^*_{\Sigma'}\xi|_{\Sigma'\cap U_p} = f(x_p)dx_p$. Therefore, $\nabla_{\mathcal{F}}s^*_{\Sigma'}\xi|_{\Sigma'\cap U_p}$ for all $p \in \sigma$ and so $\nabla_{\mathcal{F}}s^*_{\Sigma'}\xi = 0$. 
\end{proof}

Now that the parallel transport on $G$ has been studied, we can show that the image of $\gamma$ defined in (\ref{gammamapbtodiscs}) will be contained in $Discs^{Ram}_{t_0}$. This fact will be useful in comparing the parallel transport on $W^{Ram}\rightarrow Discs^{Ram}$ with the parallel transport on $G\rightarrow \mathcal{B}$.
\begin{lemma}
Suppose that $\{\epsilon_{\alpha\in Ram}\}, \{M_{\alpha\in Ram}\}, \mathcal{U}_{Ram}$ and $\mathcal{B}_{\Sigma_0}$ satisfies the Condition \ref{howtochoosebsigma0condition} then the image of $\gamma : \mathcal{B}_{\Sigma_0} \hookrightarrow Discs^{Ram}$ is contained in $Discs^{Ram}_{t_0}$. In other words, we have
\begin{equation}\label{gammamapdefinition}
    \gamma : \mathcal{B}_{\Sigma_0} \hookrightarrow Discs^{Ram}_{t_{0}} \hookrightarrow Discs^{Ram}.
\end{equation}
\end{lemma}
\begin{proof}
Part 1. and 2. of the Condition \ref{howtochoosebsigma0condition} ensures that the map $\gamma : \mathcal{B}_{\Sigma_0} \rightarrow Discs^{Ram}$ is well-defined. In other words, we have $\bar{M}^2_\alpha - M^2_\alpha > |a_{\alpha}(\Sigma) - a_{\alpha}(\Sigma_0)|$ for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ where $\sum_{k=0}^\infty b_{k\alpha}(\Sigma)z_\alpha^k$ converges for $|z_\alpha| < \bar{M}_\alpha$. We are going show that Part 3. of the Condition \ref{howtochoosebsigma0condition} implies that $\epsilon_\alpha^2 > |a_\alpha(\Sigma) - a_\alpha(\Sigma_0)|$ for all $[\Sigma] \in \mathcal{B}_{\Sigma_0}$, then the lemma follows.

For any ramification point $r_\alpha, \alpha \in Ram$ there exists a holomorphic differential form $\omega\in \Gamma(\Sigma_0, \Omega^1_{\Sigma_0}) \subset G_{\Sigma_0}$ such that $\omega(r_\alpha) \neq 0$. Let $i_\alpha(\omega) = \sum_{k=1}\omega_{\alpha, k}z^k_\alpha \frac{dz_\alpha}{z_\alpha} \in T_0L^{M_\alpha}_{Airy}\subset W^{\epsilon_\alpha, M_\alpha}_{t_\alpha(\Sigma_0)}$. Using the fact that $x_\alpha = a_\alpha(\Sigma) + z^2_\alpha$ on $\Sigma\cap U_\alpha$ and $x_\alpha = a_\alpha(\Sigma_0) + z^2_\alpha$ on $\Sigma_0\cap U_\alpha$, it follows that 
\begin{equation*}
    \omega(z_\alpha)|_{\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}} = \sum_{k=1}^\infty (\omega_i)_{\alpha, k}\left(\sqrt{x_\alpha - a_\alpha(\Sigma_0)}\right)^{k-1}d\sqrt{x_\alpha - a_\alpha(\Sigma_0)}
\end{equation*}
implies 
\begin{equation}\label{sstarofxionsigma}
    s^*_{\Sigma}\omega(z_\alpha)|_{\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}} = \sum_{k=1}^\infty (\omega_i)_{\alpha, k}\left(\sqrt{z^2_\alpha + a_\alpha(\Sigma) - a_\alpha(\Sigma_0)}\right)^{k-1}d\sqrt{z^2_\alpha + a_\alpha(\Sigma) - a_\alpha(\Sigma_0)}.
\end{equation}
By part 3. of the Condition \ref{howtochoosebsigma0condition} we have that $s^*_{\Sigma}\omega$ is holomorphic on $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha} \subset \Sigma$. For the expression in (\ref{sstarofxionsigma}) to be holomorphic on $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha} \subset \Sigma$ we must either have $\epsilon_\alpha^2 > |a_\alpha(\Sigma) - a_\alpha(\Sigma_0)|$ or that $\omega_{\alpha, k} = 0$ for all $k$ odd and for all $\alpha \in Ram$. But the latter option is not possible since $\omega(r_\alpha) \neq 0$.
\end{proof} 

\subsection{Comparison of vector bundles $G\rightarrow \mathcal{B}_{\Sigma_0}$, $\mathcal{H}\rightarrow \mathcal{B}$ and $W^{Ram}\rightarrow Discs^{Ram}$}
So far we have introduced 2 covariantly constant flat (weak) symplectic vector bundles $(\mathcal{H}\rightarrow \mathcal{B},\Omega_{\mathcal{H}}, \nabla_{GM})$, $(W^{Ram}\rightarrow Discs^{Ram}, \Omega, \nabla)$ and a flat coisotropic vector bundle $(G\rightarrow \mathcal{B}_{\Sigma_0}, \nabla_{\mathcal{F}})$. In the following we summarize how they are related.

\begin{proposition}\label{ghwproposition}
The morphisms $[.] : G\rightarrow \mathcal{H}$ and $i : G\rightarrow W^{Ram}$ of vector bundles are compatible with connections in the sense that
\begin{enumerate}
    \item $i(\nabla_{\mathcal{F}}\xi) = \gamma^*\nabla i(\xi)$
    \item $[\nabla_{\mathcal{F}}\xi] = \nabla_{GM}[\xi]$
\end{enumerate}
for any section $\xi \in \Gamma(\mathcal{B}_{\Sigma_0}, G)$. Moreover, they are compatible with parallel transports in the sense that
\begin{enumerate}
    \setcounter{enumi}{2}
    \item $i(s^*_{\Sigma'}\xi_{\Sigma}) = \sum_{\alpha \in Ram}[\alpha]\otimes\exp((a(\Sigma') - a(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}})i_\alpha(\xi_{\Sigma})$
    \item $[s^*_{\Sigma'}\xi_\Sigma] = \Gamma_{[\Sigma]}^{[\Sigma']}[\xi_{\Sigma}]$
\end{enumerate}
for any vector in the fiber $\xi_\Sigma \in G_\Sigma$ at $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ and $[\Sigma'] \in \mathcal{B}_{\Sigma_0}$ satisfying the condition of Lemma \ref{sstaroperatorlemma}. 
\end{proposition}
\begin{proof}
\begin{enumerate}
\item
Let $\xi \in \Gamma(\mathcal{B}_{\Sigma_0},G)$ and let us examine $\nabla_{\mathcal{F}}\xi$ on $\Sigma\cap U_\alpha \subset \Sigma$. Working in the standard local coordinates we can write $\xi_\Sigma = \xi_\alpha(z_\alpha,u)dz_\alpha$. Using the fact that $x_\alpha = a_\alpha(\Sigma) + z^2_\alpha$, we have $\frac{\partial z_\alpha}{\partial u^k}|_{x_\alpha = const} = -\frac{1}{2z_\alpha}\frac{\partial a_\alpha(\Sigma)}{\partial u^k}$ and so
\begin{align*}
    i_\alpha (\nabla_{\mathcal{F}}\xi_\Sigma)(z_\alpha) &= i_\alpha\left(\sum_{k=1}^gdu^k\left(\left(\frac{\partial}{\partial u^k}\Big|_{z_\alpha - const}\xi_\alpha - \frac{1}{2z_\alpha}\frac{\partial a_\alpha(\Sigma)}{\partial u^k}\frac{\partial}{\partial z_\alpha}\xi_\alpha\right)dz_\alpha + \xi_\alpha d\left(\frac{1}{2z_\alpha}\frac{\partial a_\alpha(\Sigma)}{\partial u^k}\right)\right)\right)\\
    &= \sum_{k=1}^g du^k\left(\frac{\partial}{\partial u^k} -  \frac{\partial a_\alpha(\Sigma)}{\partial u^k}\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)i_\alpha(\xi)_{t_\alpha(\Sigma)} = \gamma^*\nabla i_\alpha(\xi)_{t_\alpha(\Sigma)}(z_\alpha)
\end{align*}
for every $\alpha \in Ram$. It follows that $i(\nabla_{\mathcal{F}}\xi) = \gamma^*\nabla i(\xi)$ as claimed.
\item
Again, let $\xi \in \Gamma(\mathcal{B}_{\Sigma_0}, G)$. Let $[C]\in H_1(\Sigma,\mathbb{C})$ be any homology class represented by a path $C$ in $\Sigma$. Dissecting $C$ into closed segments $C_i, i = 1,...,N_C$ such that $C_i \subset U_{p}$ for some $p \in\sigma$. Then applying Leibniz integral rule on each section $C_i, i = 1,...,N_C$ of the path $C$ we have
\begin{align*}
    \oint_C \nabla_{\mathcal{F}}\xi_\Sigma &= \sum_{i=1}^{N_C}\int_{C_i}\sum_{k=1}^gdu^k\frac{\partial}{\partial u^k}\Big|_{x_{p_i} = const}(\xi_\Sigma|_{\Sigma \cap U_{p_i}}) = \sum_{i=1}^{N_C}\sum_{k=1}^gdu^k\frac{\partial}{\partial u^k}\int_{C_i}\xi_\Sigma|_{\Sigma\cap U_{p_i}}\\
    &= \sum_{k=1}^gdu^k\frac{\partial}{\partial u^k}\sum_{i=1}^{N_C}\int_{C_i}\xi_\Sigma|_{\Sigma\cap U_{p_i}} = \sum_{k=1}^gdu^k\frac{\partial}{\partial u^k}\oint_C\xi_{\Sigma}.
\end{align*}
This is equivalent to $[\nabla_{\mathcal{F}}\xi] = \nabla_{GM}[\xi]$.
\item Let $\xi_\Sigma \in G_\Sigma$ and let us write $\xi_\Sigma$ on $\Sigma \cap U_\alpha \subset \Sigma$ in the standard local coordinates as $\xi_\Sigma = \xi_\alpha(z_\alpha)dz_\alpha$. Recall that the local coordinates of $S$ on $U_\alpha$ are $(x_\alpha, y_\alpha)$ and the foliation $\mathcal{F}$ is given by $x_\alpha = const$, so we have $s^*_{\Sigma'}x_\alpha = x_\alpha$. Using the fact that $x_\alpha = a_\alpha(\Sigma) + z^2_\alpha$ on $\Sigma\cap U_\alpha$ and $x_\alpha = a_\alpha(\Sigma') + z^2_\alpha$ on $\Sigma'\cap U_\alpha$, we have
\begin{equation*}
    \xi_\Sigma(z_\alpha) = \xi_\alpha(z_\alpha)dz_\alpha = \xi_\alpha\left(\sqrt{x_\alpha - a_\alpha(\Sigma)}\right)d\sqrt{x_\alpha - a_\alpha(\Sigma)}
\end{equation*}
and
\begin{align*}
    s^*_{\Sigma'}\xi_{\Sigma}(z_\alpha) &= \xi_\alpha\left(\sqrt{x_\alpha - a_\alpha(\Sigma)}\right)d\sqrt{x_\alpha - a_\alpha(\Sigma)}\\
    &= \xi_\alpha\left(\sqrt{z^2_\alpha + a_\alpha(\Sigma') - a_\alpha(\Sigma)}\right)d\sqrt{z^2_\alpha + a_\alpha(\Sigma') - a_\alpha(\Sigma)} = \exp\left((a_\alpha(\Sigma') - a_\alpha(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)(\xi_\Sigma)
\end{align*}
By construction, $s^*_{\Sigma'}\xi_{\Sigma}$ is holomorphic on $\mathbb{A}_{\alpha,\bar{\epsilon}_\alpha,\bar{M}_\alpha} \subset \Sigma'$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha < M_\alpha < \bar{M}_\alpha$ and it can be represented by a Laurent series converging on $\mathbb{A}_{\alpha,\bar{\epsilon}_\alpha,\bar{M}_\alpha}$. Repeating the above for each ramification point $\alpha \in Ram$ and perform a Laurent series expansion, the claimed formula follows.
\item Since $(s_{\Sigma'})_* : H_1(\Sigma', \mathbb{C})\rightarrow H_1(\Sigma,\mathbb{C})$ is an isomorphism mapping $A, B$-periods on $\Sigma'$ to $A, B$-periods on $\Sigma$ then $[s^*_{\Sigma'}\xi_{\Sigma}] = \Gamma^{[\Sigma']}_{[\Sigma]}[\xi_\Sigma]$ follows straightforwardly from Lemma \ref{integralofparalleltransportlemma}.
\end{enumerate}
\end{proof}

\subsection{Relations to the residue constraints}

Let us define $\phi \in \Gamma(\mathcal{B}_{\Sigma_0},T^*\mathcal{B}\otimes G)$. For any point $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ and vector $v = \sum_{k=1}^gv_k\frac{\partial}{\partial u_k} \in T_{[\Sigma]}\mathcal{B}_{\Sigma_0}$, $\phi_{\Sigma}(v) \in \Gamma(\Sigma,\Omega^1_{\Sigma}) \subset G_{\Sigma}$ is given in the local coordinates on $U_p$ by
\begin{align*}\label{phiBvalue}
    \phi_{\Sigma}(v)|_{\Sigma\cap U_p} &= \Omega_S\left(\sum_{k=1}^g v_k\left(\frac{\partial x_p}{\partial u_k}\frac{\partial}{\partial x_p} + \frac{\partial y_p}{\partial u_k}\frac{\partial}{\partial y_p}\right),.\right)\Big|_{\Sigma\cap U_p}\\
    &= \Omega_S\left(\sum_{k=1}^g v_k \frac{\partial y_p}{\partial u_k}\frac{\partial}{\partial y_p},.\right)\Big|_{\Sigma\cap U_p} = -\sum_{k=1}^gv_k\frac{\partial y_p}{\partial u_k}dx_p\Big|_{\Sigma\cap U_p} = -\iota_v\nabla_{\mathcal{F}}(y_pdx_p)|_{\Sigma\cap U_p}.\numberthis
\end{align*}
We compare this to $\phi_{\alpha} \in \Gamma(Discs^{\epsilon_\alpha, M_\alpha}_{t_{0\alpha}}, Hom(TDiscs^{\epsilon_\alpha, M_\alpha}_{t_{0\alpha}},W^{\epsilon_\alpha,M_\alpha}))$ previously studied, which we can re-derive here by taking the derivative keeping $x_\alpha = const$. Given $t_\alpha \in Discs^{\epsilon_\alpha, M_\alpha}_{t_0\alpha}, t_\alpha = (x_\alpha = z^2_\alpha + a_\alpha, y_\alpha = \sum_{k=0}^\infty b_{k\alpha}y_\alpha^k)$ and vector $v_\alpha = A\frac{\partial}{\partial a_\alpha} + \sum_{k=0}^\infty B_k\frac{\partial}{\partial b_{k\alpha}} \in T_{t_\alpha}Discs^{\epsilon_\alpha, M_\alpha}_{t_{0\alpha}}$ then using $\frac{\partial z_\alpha}{\partial a_\alpha}|_{x_\alpha = const} = -\frac{1}{2z_\alpha}$ we have 
\begin{equation*}
    \phi_{\alpha,t_\alpha}(v_\alpha) = \Omega_S\left(\left(A\frac{\partial y_\alpha}{\partial a_\alpha} + \sum_{k=0}^\infty B_k\frac{\partial y_\alpha}{\partial b_{k\alpha}}\right)\frac{\partial}{\partial y_\alpha},.\right) = -\left(\sum_{k = 0}^\infty B_kz^k_\alpha - \frac{A}{2z_\alpha}\sum_{k=1}^\infty kb_{k\alpha}z^{k-1}_\alpha\right)dx_\alpha.
\end{equation*}
Setting $t_\alpha = t_\alpha(\Sigma) = \gamma_\alpha(\Sigma)$ and $v_\alpha = d\gamma(v) = \sum_{k=1}^g \left(v_k\frac{\partial a_\alpha(\Sigma)}{\partial u^k}\frac{\partial}{\partial a_\alpha} + \sum_{l=0}^\infty v_k\frac{\partial b_{l\alpha}(\Sigma)}{\partial u^k}\frac{\partial}{\partial b_{l\alpha}}\right)$ shows that $i_\alpha \phi_\Sigma = \gamma^*\phi_\alpha = \phi_\alpha \circ d\gamma$. We define $\phi := \prod_{\alpha \in Ram}\phi_\alpha \in \Gamma(Discs^{Ram}_{t_0}, Hom(TDiscs^{Ram}_{t_0},W^{Ram}))$. Evidently, we also have $[\phi_\Sigma] = \pmb{\phi}_\Sigma$ as defined in Section \ref{deformationofcurvessection}. We can summarize this discussion by the following commutative diagram
\begin{equation*}
    \begin{tikzcd}
    T_{[\Sigma]}\mathcal{B}_{\Sigma_0}\arrow{r}\arrow[bend left, hookrightarrow]{rr}{\pmb{\phi}_\Sigma}& \Gamma(\Sigma, \Omega^1_\Sigma)\arrow[hookrightarrow]{r}& \mathcal{H}_\Sigma \arrow{r}{\cong} & G_\Sigma/G^\perp_\Sigma \\ \\
    T_{[\Sigma]}\mathcal{B}_{\Sigma_0}\arrow{r}\arrow[bend left, hookrightarrow]{rr}{\phi_\Sigma}\arrow{uu}{\cong}\arrow{dd}{d\gamma}& \Gamma(\Sigma, \Omega^1_\Sigma)\arrow[hookrightarrow]{r}& G_\Sigma\arrow{uu}{[.]}\arrow{dd}{i} \\ \\
    T_{t(\Sigma)}Discs^{Ram}_{t_0}\arrow{r}\arrow[bend left, hookrightarrow]{rr}{\phi_{t(\Sigma)}}& T_0L^{Ram}_{Airy}\arrow[hookrightarrow]{r}& W^{Ram}_{t(\Sigma)} \arrow{r}{\cong} & W^{Ram}_{Airy}
    \end{tikzcd}
\end{equation*}
Since $d_\nabla\phi_{\alpha} = 0$ and $W^{\epsilon_\alpha, M_\alpha}\rightarrow Discs^{M_\alpha}_{t_0}$ is a flat vector bundle we have a section $\theta_\alpha \in \Gamma(Discs^{M_\alpha}_{t_0}, W^{\epsilon_\alpha, M_\alpha})$ such that $d_\nabla \theta_\alpha = \phi_\alpha$ where $\theta_{\alpha, t_\alpha} = -y_\alpha dx_\alpha$. Similarly, because $d_{\nabla_{\mathcal{F}}}\phi = 0$ and $G\rightarrow \mathcal{B}_{\Sigma_0}$ is a flat vector bundle, there exists $\theta \in \Gamma(\mathcal{B}_{\Sigma_0}, G)$ such that $\nabla_{\mathcal{F}} \theta = \phi$. So $\theta_\Sigma$ is a holomorphic differential form on $\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}$ for some $\bar{\epsilon}_\alpha < \epsilon_\alpha$, $\oint_{\partial\bar{\mathbb{D}}_{\alpha, \epsilon_\alpha}}\theta_\Sigma = 0$ and any infinitesimal variation of $\theta_\Sigma$ in moduli space directions produce a holomorphic form on $\Sigma$. Also, by taking cohomology class and apply Proposition \ref{ghwproposition}, we find that $\nabla_{GM}[\theta_{\Sigma}] = [\nabla_{\mathcal{F}}\theta_\Sigma] = [\phi_\Sigma] = \pmb{\phi}_{\Sigma}$. So we may define $\pmb{\theta} := [\theta]$. 

From (\ref{phiBvalue}) we must have $\theta_\Sigma|_{\Sigma\cap U_p} = -(y_p + f_p(x_p))dx_p|_{\Sigma\cap U_p}$ where $f_p(x_p)dx_p$ is an integration constant. On $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha} \subset \Sigma\cap U_\alpha$ the integration constant can be written as $f_\alpha(x_\alpha)dx_\alpha = f_\alpha(z_\alpha^2 + a_\alpha(\Sigma))d(z_\alpha^2)$ where $x_\alpha \mapsto f_\alpha(x_\alpha)$ need not be single-valued as long as $z_\alpha \mapsto f_\alpha(z_\alpha^2 + a_\alpha(\Sigma))$ is single-valued on $\mathbb{A}_{\alpha,\epsilon_\alpha,M_\alpha}$. For example, we might have $f_\alpha(x_\alpha) = \sqrt{x_\alpha - a_\alpha(\Sigma_0)} = \sqrt{z^2_\alpha + a_\alpha(\Sigma) - a_\alpha(\Sigma_0)}$ which is a well-defined function on $\mathbb{A}_{\alpha,\epsilon_\alpha, M_\alpha}$.

Let us show explicitly how $\theta \in \Gamma(\mathcal{B}_{\Sigma_0}, G)$ such that $\nabla_{\mathcal{F}}\theta = \phi$ can be constructed. Let us write $y_p(x_p;\Sigma)dx_p := y_pdx_p|_{\Sigma\cap U_p}$ for each $p \in \sigma$. In other words, $\{(x_p, y(x_p;\Sigma)) \in U_p \subset S\ |\ x_p \in x_p(\Sigma\cap U_p)\}$ is the graph of $\Sigma \cap U_p$. Then we define $\theta_\Sigma$ on each open subset $\Sigma\cap U_p$ by
\begin{equation*}
    \theta_\Sigma|_{\Sigma\cap U_p} := -y_p(x_p;\Sigma)dx_p + y_p(x_p;\Sigma_0)dx_p.
\end{equation*}
We need to check that $\theta_\Sigma|_{\Sigma\cap U_p}$ for each $p \in \sigma$ patch together to form a well defined holomorphic function on $\Sigma\setminus \cup_{\alpha \in Ram}\bar{\mathbb{D}}_{\alpha, \bar{\epsilon}_\alpha}$. Using the coordinates transformation on $U_p\cap U_{p'}$ between $(x_p, y_p)$ and $(x_{p'}, y_{p'})$ as given in (\ref{coordtransfpandpprime}), we find that $x_{p'} = F_{p'}(x_p)$ and
\begin{equation*}
    y_{p'}(x_{p'};\Sigma) = \frac{y_{p}(F^{-1}_{p'}(x_{p'});\Sigma)}{F'_{p'}(F^{-1}(x_{p'}))} - G'_{p'}(F^{-1}(x_{p'})), \qquad y_{p'}(x_{p'};\Sigma_0) = \frac{y_{p}(F^{-1}_{p'}(x_{p'});\Sigma_0)}{F'_{p'}(F^{-1}(x_{p'}))} - G'_{p'}(F^{-1}(x_{p'})).
\end{equation*}
This means
\begin{align*}
    \left(\theta_{\Sigma}|_{\Sigma\cap U_{p'}}\right)|_{\Sigma\cap U_{p}\cap U_{p'}} &= -y_{p'}(x_{p'};\Sigma)dx_{p'} + y_{p'}(x_{p'};\Sigma_0)dx_{p'}\\
    &= -\left(\frac{y_{p}(F^{-1}_{p'}(x_{p'});\Sigma)}{F'_{p'}(F^{-1}(x_{p'}))} - G'_{p'}(F^{-1}(x_{p'}))\right)dx_{p'} + \left(\frac{y_{p}(F^{-1}_{p'}(x_{p'});\Sigma_0)}{F'_{p'}(F^{-1}(x_{p'}))} - G'_{p'}(F^{-1}(x_{p'}))\right)dx_{p'}\\
    &= -\left(\frac{y_{p}(x_p;\Sigma)}{F'_{p'}(x_p)} - G'_{p'}(x_p)\right)dF(x_p) + \left(\frac{y_{p}(x_p;\Sigma_0)}{F'_{p'}(x_p)} - G'_{p'}(x_p)\right)dF(x_p)\\
    &= -y_p(x_p;\Sigma)dx_p + y_p(x_p;\Sigma_0)dx_p\\
    &= \left(\theta_{\Sigma}|_{\Sigma\cap U_{p}}\right)|_{\Sigma\cap U_{p}\cap U_{p'}}.
\end{align*}
Therefore, we have well-defined function $\theta_\Sigma$ on $\cup_{p \in \sigma}U_p \supset \Sigma\setminus \cup_{\alpha \in Ram}\mathbb{D}_{\alpha, \epsilon_\alpha}$. In particular, $\theta_\Sigma$ we have so far is well-defined on the annulus $\mathbb{A}_{\alpha, \epsilon_\alpha, M_\alpha}$ and can be written as 
\begin{equation*}
    i_\alpha\theta_\Sigma(z_\alpha) = -\theta_{t(\Sigma)} + \exp((a_\alpha(\Sigma) - a_\alpha(\Sigma_0))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}})\theta_{t(\Sigma_0)}
\end{equation*}
which contains no $\frac{dz_\alpha}{z_\alpha}$ according to Lemma \ref{expoperatorlemma} and so $\oint_{\partial\bar{\mathbb{D}}_{\alpha,\epsilon_\alpha}}\theta_\Sigma = 0$. The exponential operator appeared because we are comparing $\theta_{t(\Sigma)}$ with $\theta_{t(\Sigma_0)}$ on the same foliation leaf $x_\alpha = const$ but $x_\alpha = z^2_\alpha + a_\alpha(\Sigma)$ on $\Sigma$ and $x_\alpha = z^2_\alpha + a_\alpha(\Sigma_0)$ on $\Sigma_0$.

We will embed the neighbourhood $\mathcal{B}_{\Sigma_0}$ of $[\Sigma_0] \in \mathcal{B}$ into the fiber $G_{\Sigma_0}$ in the same way we did in Section \ref{deformationofcurvessection}. The embedding map $\Phi_{\Sigma_0} : \mathcal{B}_{\Sigma_0} \rightarrow G_{\Sigma_0}$ is given by sending the zero vector $0_{\Sigma} \in G_{\Sigma}$ at $[\Sigma] \in \mathcal{B}_{\Sigma_0}$ into $G_{\Sigma_0}$ at $[\Sigma_0]\in \mathcal{B}_{\Sigma_0}$ via parallel transport using the connection $\nabla_{\mathcal{F}} + \phi$. Since $\nabla_{\mathcal{F}}\theta = \phi$, the parallel transport of $0_\Sigma$ from $[\Sigma] \in \mathcal{B}_{\Sigma'}$ to $[\Sigma'] \in \mathcal{B}$ using $\nabla_{\mathcal{F}} + \phi$ is path-independent and it is uniquely given by 
\begin{equation*}
    v_{\Sigma}(\Sigma') = -\theta_{\Sigma'} + s^*_{\Sigma'}\theta_{\Sigma}.
\end{equation*}
Therefore,
\begin{equation*}
    \Phi_{\Sigma_0}(\Sigma) := v_{\Sigma}(\Sigma_0) = -\theta_{\Sigma_0} + s^*_{\Sigma_0}\theta_\Sigma \in G_{\Sigma_0}.
\end{equation*}
Finally, we have the following proposition which is essentially a version of Proposition 7.1.2 of \cite{kontsevich2017airy}.
\begin{proposition}
The embedding $\Phi_{\Sigma_0} : \mathcal{B}_{\Sigma_0} \rightarrow G_{\Sigma_0}$ satisfies $[\Phi_{\Sigma_0}(\Sigma)] = \pmb{\Phi}_{\Sigma_0}(\Sigma)$ and $i(\Phi_{\Sigma_0}(\Sigma)) = \Phi_{t_0}\circ\gamma(\Sigma) = \Phi_{t_0}(t(\Sigma))$, so $(\mathbf{a})$ and $(\mathbf{b})$ squares in the diagram are commutative.
Moreover, by choosing the local coordinates $(x_\alpha, y_\alpha)$ on $U_\alpha$ such that $\gamma_\alpha(\Sigma_0) = (x_\alpha = z^2_\alpha, y_\alpha = z_\alpha)$ the triangle $(\mathbf{c})$ in the diagram is also commutative
\begin{equation*}
    \begin{tikzcd}
    \mathcal{B}_{\Sigma_0}\arrow[hookrightarrow]{rr}{\pmb{\Phi}_{\Sigma_0}} && \mathcal{H}_{\Sigma_0} \arrow{r}{\cong} & G_{\Sigma_0}/G^\perp_{\Sigma_0} \\ & (\mathbf{a}) \\
    \mathcal{B}_{\Sigma_0}\arrow[hookrightarrow]{rr}{\Phi_{\Sigma_0}}\arrow{uu}{\cong}\arrow{dd}{d\gamma}&& G_{\Sigma_0}\arrow{uu}{[.]}\arrow{dd}{i} \\ & (\mathbf{b}) \\
    Discs^{Ram}_{t_0}\arrow[hookrightarrow]{rr}{\Phi_{t_0}}\arrow{rdd}&& W^{Ram}_{t_0} \arrow{r}{\cong} & W^{Ram}_{Airy} \\ & (\mathbf{c}) \\
    & L^{Ram}_{Airy}\arrow[hookrightarrow]{ruu}
    \end{tikzcd}
\end{equation*}
\end{proposition}
\begin{proof}
This is mostly an application of Proposition \ref{ghwproposition}. We have
\begin{equation*}
    [\Phi_{\Sigma_0}(\Sigma)] = -[\theta_{\Sigma_0}] + [s^*_{\Sigma_0}\theta_{\Sigma}] = -[\theta_{\Sigma_0}] + \Gamma^{[\Sigma_0]}_{[\Sigma]}[\theta_{\Sigma}] = -\pmb{\theta}_{\Sigma_0} + \Gamma^{[\Sigma_0]}_{[\Sigma]}\pmb{\theta}_{\Sigma} = \pmb{\Phi}_{\Sigma_0}
\end{equation*}
and so $(\mathbf{a})$ is commutative.
Similarly, 
\begin{align*}
    i(\Phi_{\Sigma_0}(\Sigma)) &= -i(\theta_{\Sigma_0}) + i(s^*_{\Sigma_0}\theta_{\Sigma})\\
    &= -i(\theta_{\Sigma_0}) + \sum_{\alpha \in Ram}[\alpha] \otimes \exp\left((a_\alpha(\Sigma_0) - a_\alpha(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)i_\alpha(\theta_\Sigma)\\
    &= \sum_{\alpha \in Ram}[\alpha]\otimes \Big(-\theta_{t_\alpha(\Sigma_0)} + f_\alpha(z_\alpha^2 + a_\alpha(\Sigma_0))d(z_\alpha^2)\\
    &\qquad\qquad\qquad\qquad + \exp\left((a_\alpha(\Sigma_0) - a_\alpha(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)\left(\theta_{t_\alpha(\Sigma)} - f_\alpha(z_\alpha^2 + a_\alpha(\Sigma))d(z_\alpha^2)\right)\Big)\\
    &= \sum_{\alpha \in Ram}[\alpha]\otimes \Big(-\theta_{t_\alpha(\Sigma_0)} + f_\alpha(z_\alpha^2 + a_\alpha(\Sigma_0))d(z_\alpha^2)\\
    &\qquad\qquad\qquad\qquad + \exp\left((a_\alpha(\Sigma_0) - a_\alpha(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)\theta_{t_\alpha(\Sigma)} - f_\alpha(z_\alpha^2 + a_\alpha(\Sigma_0))d(z_\alpha^2)\Big)\\
    &= \sum_{\alpha \in Ram}[\alpha]\otimes \left(-\theta_{t_\alpha(\Sigma_0)} + \exp\left((a_\alpha(\Sigma_0) - a_\alpha(\Sigma))\mathcal{L}_{\frac{1}{2z_\alpha}\partial_{z_\alpha}}\right)\theta_{t_\alpha(\Sigma)}\right)\\
    &= \Phi_{t_0}(t(\Sigma)) = \Phi_{t_0}\circ\gamma(\Sigma)
\end{align*}
and so $(\mathbf{b})$ is commutative. Lastly, if $\gamma_\alpha(\Sigma_0) = (x_\alpha = z^2_\alpha, y_\alpha = z_\alpha)$ then it follows from Proposition \ref{phiembeddiscsinwproposition} that $\text{im} \Phi_{t_0} \subset L^{Ram}_{Airy}$ which shows that $(\mathbf{c})$ is commutative.
\end{proof} 

==> old.tex <==
\section{Airy structures}  \label{quadlag} 
In this section we give the formulation of topological recursion due to Kontsevich and Soibelman \cite{KSoAir}. 
    
\subsection{Tate spaces}
    
    %why tate - for the dual?
    
    We outline the algebraic background needed to define an \emph{Airy structure}, on an infinite dimensional \emph{Tate space} \( W \), over a field \( \mathbf{k}\) of characteristic zero with discrete topology, from \cite{KSoAir}. Tate spaces are a model for an infinite dimensional symplectic vector space. Tate spaces are necessary for topological recursion. This is because the corresponding Airy structure is on the space of meromorphic differentials over a curve, which is infinite dimensional. Giving this space discrete topology allows for taking a  (topological) dual. In this case, this also gives the stronger property \(W \simeq W^*\). 
    
    An Airy structure is equivalent to a \emph{Lagrangian} subvariety in an infinite dimensional \emph{symplectic vector space} or Tate space. The input to generate an Airy structure is a topological vector space \(V\), equipped with the discrete topology, over \( \mathbf{k}\).
    There is the additional requirement that \(V \simeq (V^*)^*\), (where \(*\) denotes topological dual). This gives \(V^*\) linearly compact topology \cite{drinfeld_tate}. 
    Then this gives the \emph{Tate} space \(W = V \oplus V^* \simeq V \oplus L\) \cite{drinfeld_tate} which has a natural symplectic structure. 
    
    Define \emph{Darboux} coordinates \(x^k \) indexed by \( \mathbb{N}\) on \(V^* \simeq L\), and note \( x^k \in (V^*)^* \simeq V\). Likewise there are coordinates \(y_k\) on \(V\), and also \(y_k \in  V^* \simeq L\).  \(x\) and \(y\) can now also be treated as formal variables in a coordinate ring, via the identification \[ \mathrm{Sym}(W^*) \simeq \mathbf{k}[W] := \mathbf{k}[x^{\sbt},y_{\sbt}] := \lim_n \, \mathbf{k}[x^1, \dots x^{n},y_{1}, \dots y_n],\] 
    where \( \mathbf{k}[x^{\sbt},y_{\sbt}]\) is understood as a ring of polynomials in infinite variables but bound in degree, \(\mathrm{lim}\) is the projective limit.

    Additionally there is a natural isomorphism between completed tensor products, and a ring of formal power series in infinite variables 
    \[\widehat{\mathrm{Sym}}(W^*) \simeq \mathbf{k}\llbracket x^{\sbt} , y_{\sbt} \rrbracket := \mathbf{k}\llbracket W \rrbracket.  \]
    Where \( \mathbf{k}\llbracket W \rrbracket \) is given by completion at the maximal ideal \( \langle x^{\sbt}, y_{\sbt} \rangle \). Note \( \mathbf{k}[ W ]\) is an Artin ring (descending ideal condition) with \(I\)-adic topology. 
    
    The symplectic structure on \(W\) as a vector space, lifts naturally to a \emph{Poisson bracket} on \( \mathbf{k}[W]\) and on the completion \(\mathbf{k}\llbracket W \rrbracket\). The Poisson bracket is a map \( \{ {\sbt}, {\sbt}\}: \mathbf{k}[ W]  \times \mathbf{k}[ W ] \rightarrow \mathbf{k}[ W ]\), defined by the coordinates, \( \{ y_j,x^i\} := \delta^i_j \), \( \{x^i,x^j\} := 0\) and \( \{ y_i, y_j \}: = 0\), and extending to polynomials and formal series via Leibniz. This gives \( k[W]\) the structure of a Lie algebra.
    
    \begin{example}
    Consider \(V\) as the space of global meromorphic differentials with zero \(A\) periods given the discrete topology.
    \end{example}
    
    %Then a \emph{symplectic} (0,2)-form on \(W\), \( \omega : \text{Der}(\mathbf{k}[W]) \times \text{Der}(\mathbf{k}[W]) \rightarrow \mathbf{k}[W] \) is defined, so that for  derivations \(X_f =\{ f, \sbt \} \), where \(f \in \mathbf{k}[W] \), such that \( \omega(X_f,X_g) := \{ f,g\} \). Therefore \(W\) then has the structure of a (strong) symplectic (topological) vector space. 
    %canonical isomorphism / remark treat x/y as basis
    %%%Airy structure
    Recall \(G \subset W\) is \emph{coisotropic} if the corresponding subalgebra of functions vanishing on \(G\), \( \mathbf{k}[ G ]\), is closed under the Poisson bracket.

    
\subsection{Airy structures}
    
    Consider an infinite collection of quadratic Hamiltonians, effectively polynomials, \( H_i \in \mathbf{k}[ W ] \) where
    \[ H_i=-y_i+a_{ijk} \, x^j x^k+ 2 b_{ij }^{k } \, x^j y_k +c_{i}^{ jk}\,y_j y_k, \quad i,j,k \in \mathbb{N}.\] 
    
    \begin{defn}[Airy structure]
    An \emph{Airy structure} is a choice of coefficients \((a_{ijk},b_{ij}^k,c_i^{jk})\) satisfying the constraint that the \(H_i\) form a Lie algebra \( \mathfrak{g}\) with structure constants \(g_{ij}^k\), given by the closure of the Poisson bracket from \(\mathbf{k}[W]\):
    \[ \{ H_i, H_j \} = g_{ij}^k H_k. \]
    Explicitly the coefficients must satisfy:
    \begin{align*}
       2 \left(  b_{ji}^k - b_{ij}^k \right) &= g_{ij}^k,\\
       4\left( a_{jks} b_{it}^k -  a_{iks} b_{jt}^k \right) &=  g_{ij}^k  a_{kst}, \\
       4\left(  a_{jks} c_i^{k t} -  a_{ik s} c_j^{k t} +  b_{is}^k b_{jk}^t  -  b_{ik}^t b_{js}^k \right) & = 2 g_{ij}^k b_{k s t}^k, \\ 
       4 \left( b_{jk}^s c_i^{kt}  - b_{ik}^s c_j^{kt}\right) &= g_{ij}^k c_k^{st}.
    \end{align*}
    \end{defn}
    Necessarily \( \mathfrak{g} \simeq L\).
    
    %The coefficients of \(H_i\) can be identified with tensors on \(V\) and \(V^*\) by pairing with a basis.
    \( \mathbf{k}[W]\) has a maximal ideal \(\mathfrak{m} = \langle x^{\sbt}, y_{\sbt} \rangle\). Linearising \(H_i\) gives equations \(L_i = -y_i\). The quotient \( \mathcal{L}= \mathrm{Spec} \left( \mathbf{k}[W]/\langle H_i \rangle  \right) \) defines a subvariety in \(W\). The tangent space at \(0\) is given by \( T_0 \mathcal{L} = \mathfrak{m}/(\langle L_i \rangle  + \mathfrak{m}^2) \simeq L \).
    
    An Airy structure is equivalent to a choice of \(\mathcal{L}\) in \(W\). 

    %Either we are given a \(V\) and then there is a natural symplectic structure structure. Or we are given a symplectic space \(W\) with symplectic form, and we choose \(L\) and coordinates. Both equivalently define a \( \mathcal{L}\). Either there is a symplectic form and there is a choice of \(V\) up to isomorphism, or \(V\) is given which defines a symplectic form.
    
    
    We are interested in studying \( \mathcal{L}\) in formal neighbourhoods of the origin, via a formal germ. Corresponding to \(\mathcal{L}\) is a formal scheme \( \widehat{\mathcal{L}} \) which is given by completion of \(\mathcal{L}\) along a maximal ideal \( \mathfrak{m}\) (at zero in \(W\))).
    
    Concretely \( \widehat{\mathcal{L}} \simeq \mathrm{Spf} \left(\mathbf{k}\llbracket W \rrbracket/\langle y_i - u_{0;i}(x^{\sbt} \rangle \right)  \), where the \(u_{0;i}\) are given by solving \(H_i= 0\) for \(y_i\) as a function of the \(x^i\), so \( y_i = u_{0,i}(x^{\sbt}) \) via fixed point iteration. 
    
    \begin{remark}[Formal Germ] There are several notions of formal germ.
    
    \end{remark}
    
    \begin{example}
    Consider the conic \(-y+x^2 + 2 xy + y^2=0\). Solving for \(y\), and taking the formal expansion of the square root gives
    \( u_0(x) = x^2 + 2 x^3 + 5 x^4 + \cdots + \frac{(2n)!}{(n+1)!n!} x^{n+1}  + \cdots\). Coefficients are Catalan numbers, which count rooted binary trees.
    \end{example}

    %The tangent space to \( \mathcal{L} \) is given by setting \(y_i = 0\), which should recover \(L\).
    
    %More generally, \(\mathcal{L}\) is given by a localisation and a completion  \(  \lim_{\leftarrow} \mathbf{k}[W] / \mathcal{I}^n \), where \(\mathcal{I}\) is a Poisson ideal  \(\mathcal{I} = \langle H_i \rangle \). Specifically this gives a formal power series \( S_0 \in \mathbf{k} \llbracket x^{\sbt}\rrbracket\) which is zero on \(L\).
    
    % gauge transformations of airy structures

    In general, the formal series \(u_{0;i}\) can be constructed via the following fixed point iteration, which is equivalent to the zero genus part of Theorem 2.4.2 in \cite{KSoAir};
    \begin{align*} 
    u_{0;i}^{(0)} &= a_{ijk} x^j x^k \\
    u_{0;i}^{(n)} &= a_{ijk} x^j x^k + 2 b_{ij}^k x^j u^{(n-1)}_{0;k} + c_{i}^{jk} u^{(n-1)}_{0;j} u^{(n-1)}_{0;k}.
    \end{align*}
    Coefficients of this formal series stabilise -- which can be proven inductively. \(u_0\) starts from a cubic term. 
    
    Taking the colimit of the quotient gives \( \widehat{\mathcal{L}}\), 
    \[ \widehat{\mathcal{L}} = \underset{n}{\mathrm{colim}} \, \mathrm{Spec} \left( \mathcal{L}/\mathfrak{m}^n \right), \]
    %frac{ \mathbf{k}[ x_{\sbt} , y^{\sbt} ]}{ \langle H_i \rangle / \mathrak{m}^n } 
    via the projective limit functor. 
    
    Defining \( u_0(x^{\sbt}) = u_{0,i}(x^{\sbt}) x^i \), monomials can be identified with tensors in \( \widehat{\mathrm{Sym}}(V) \). The first few coefficients of \(u_0\) are 
    \[ \{ a_{ijk} , 2 b^k_{ij} a_{krs} , c_i^{jk} a_{jrs} a_{ktu}  +  4 b_{ij}^{k} b_{kr}^s a_{s tu} , \dots \}. \]
    
    
    \subsection{Tate spaces over a symplectic surface}
    \label{section:universal}

    % In this section, a bundle of Tate spaces are associated to curves in a symplectic surface \(X\).
    
    % Let  $(X,\omega)$ be a symplectic surface with a Lagrangian foliation $\cF$. 
    
    
    % Consider an infinite dimensional space $Coord$ parameterizing the space of tuples $(s,x,y)$, where $s \in X$ and $(x,y)$ is a formal coordinate system at the point $s$ such that the symplectic form $\omega$ is equal to $dx \wedge dy$ and the tangent bundle of the foliation $\cF$ is generated by the vector field $\partial_y$. 
    % There is a $3:1$ degree map $\pi:Coord \rightarrow Discs$ which sends a point $(s,x,y)$ to the formal disc with coordinate $z$ embedded via the assignment $z \rightarrow (x=z^2,y=z)$. The pull-back of the vector bundle $\ch_t$ defined in Section \ref{formal} is a canonically trivialized symplectic vector bundle, whose fibers are identified with the space $W = \otimes_{r \in R} W_{Airy} $, where
    % $$W_{Airy}=\mathrm{Ker}(\mathrm{Res}_z: \bc \llparenthesis z \rrparenthesis) dz \rightarrow \bc)$$
    % and $R$ denotes a divisor.
    
    % The system of equations
    % $$\mathrm{Res}_z(x^k ydx)=0, k \geq 1 \qquad \mathrm{Res}_z(x^k y^2 dx)=0, k \geq 0,$$
    % gives the formal germ of the Lagrangian \(\mathcal{L}\) of $W$.
    
    % Denote by $V^*$ the tangent space of the Lagrangian $\mathcal{L}$ at the origin and by $V$ its topological dual. This gives the decomposition $W=V \oplus V^*$.
    % By \cite[Corollary 7.2.1]{KSoAir} the vector space $V$ carries an Airy structure. 
    
    % %Therefore, the Lagrangian $\mathcal{L}$ defines a cyclic deformation quantization module which is generated by wave function $\psi=\exp \left( \sum_{g \geq 0} \hb^{g-1}\, S_g  \right)$.

    
    % In the $k$-th formal neighbourhood of $0\in W$, for each $k$, a quadratic Lagrangian $\cl$ is defined as follows.  An element $\eta$ in the $k$-th formal neighbourhood of $0\in W$ lives in $\cl$, i.e. it is annihilated by the ideal defining $\cl$, if it satisfies the following residue constraints \cite{KSoAir}.  For $(x_\alpha,y_\alpha)$ local coordinates in a neighbourhood of $\alpha\in R\subset\Sigma_0\subset X$ chosen so that $x_\alpha-y_\alpha^2=0$ defines $\Sigma_0$:
    % \begin{eqnarray}  \label{rescon1}
    % \Res_\alpha\left(y_\alpha-\frac{\eta}{dx_\alpha}\right)x_\alpha^mdx_\alpha=0,\quad m\geq 1\\
    % \Res_\alpha\left(y_\alpha-\frac{\eta}{dx_\alpha}\right)^2x_\alpha^mdx_\alpha=0,\quad m\geq 0. \label{rescon2}
    % \end{eqnarray} 
    % The condition that the differential $\Res_\alpha\eta x_\alpha^mdx_\alpha=0$ for $m\geq 0$ is equivalent to $\eta$ having skew-invariant principal part under the local involution $\sigma_\alpha$.\\
    
    %Are the residue constraints independent of the choice of local coordinates $(x_\alpha,y_\alpha)\mapsto(f(x_\alpha),y_\alpha/f'(x_\alpha)+g(x_\alpha))$?

    \subsection{Symplectic reduction}  \label{sympred}

        Consider a symplectic manifold $(M,\omega)$ that admits a proper Hamiltonian action of an abelian Lie group $G$ and an invariant moment map $\mu:M\to\mathfrak{g}^*$.  For $\xi\in\mathfrak{g}$ define the vector field on $M$ by
        $$v_{\xi}=\left.\frac{d}{dt}\right|_{t=0}\hspace{-3mm}\exp(t\xi)\cdot m.
        $$
        The moment map satisfies
        $$\omega(v_{\xi},\cdot)=d\langle\mu,\xi\rangle.
        $$
        For any regular value $a$ of $\mu$, define the symplectic quotient
        $$ M\sslash G:=\mu^{-1}(a)/G.
        $$
        Then $M\sslash G$ inherits a symplectic form (depending on $a$).
        
        Apply these ideas to a symplectic vector space $(W,\omega)$ equipped with a translation-invariant symplectic form $\omega$.  Let $U\subset W$ be an isotropic subspace, so $\omega|_{U}=0$ or equivalently $U\subset U^\perp$.  Then $U$ acts on $W$ by translations, an hence preserves $\omega$.  The moment map $\mu$ is given by the quotient map
        $$0\to U^\perp\to W\stackrel{\mu}{\to} U^*\to 0
        $$
        since $\langle\mu(m),u\rangle=\omega(u,m)$ for any $m\in W$.  Hence $U^\perp=\mu^{-1}(0)$ and the symplectic quotient is given by:
        $$ W\sslash U:=U^\perp/U.
        $$
        The symplectic form $\overline{\omega}$ on $W\sslash U$ is defined by $\overline{\omega}(\bar{v}_1,\bar{v}_2)=\omega(v_1,v_2)$ where $v_i\in U^\perp$ is any lift of $\bar{v}_i\in U^\perp/U$.  The right hand side is independent of the lift since $\omega(v_1+u,v_2)=\omega(v_1,v_2)$ for any $u\in U$.  The 2-form $\overline{\omega}$ is closed since it is translation invariant.  It is non-degenerate since $\overline{\omega}(\bar{v}_1,\bar{v}_2)=\omega(v_1,v_2)=0$ for all $\bar{v}_2$, hence all $v_2$ implies that $v_1\in U$ hence $\bar{v}_1\equiv 0$.
        
        Following \cite{KSoAir}, define the symplectic vector space
        $$ W_{\text{Airy}}=\left\{ J=\sum_{n\in\bz} J_nz^{-n}\frac{dz}{z}\mid J_0=0, \exists N \text{ such that }J_n=0,\ n>N\right\}
        $$
        with symplectic form
        $$\omega(\eta_1,\eta_2)=\Res_{z=0}f_1\eta_2,\quad df_1=\eta_1,\eta_2\in W.
        $$
        The skew-symmetric bilinear form $\omega$ is translation-invariant hence closed.  It is non-degenerate because for $J=\sum_{n\geq k} J_nz^{-n}\frac{dz}{z}\in W$, with $J_k\neq 0$, then $\omega(J,z^k\frac{dz}{z})\neq 0$.  It is easy to see that $W_{\text{Airy}}\supset L_{\text{Airy}}=\{J\mid J_n=0,n>0\}$ is a lagrangian subspace.
        
        
        
        Given a compact Riemann surface $\Sigma$, a non-empty finite subset $R\subset\Sigma$, and local coordinates $z_\alpha$ defined in a neighbourhood of $\alpha\in R$, define $W=(W_{\text{Airy}})^R$.  Each copy of $W_{\text{Airy}}$ uses the local coordinate $z_\alpha$.  The subspace $ L=(L_{\text{Airy}})^R\subset W$ is Lagrangian.  Define $G_\Sigma\subset W$ by
        $$
        G_\Sigma=\{ \eta\in H^0(\Omega^1(\Sigma-R)) \text{\ meromorphic on }\Sigma\mid\Res_{r\in R}\eta=0\}
        $$
        where we identify $G_\Sigma$ with its image under the injective map $G_\Sigma\to W$.  
        \begin{lemma}[\cite{KSoAir}]  \label{coisotropic}
        $G_\Sigma\subset W$ is coisotropic.
        \end{lemma}
        \begin{proof}
        We first show that $G_\Sigma$ and $L$ intersect transversally, i.e.
        \begin{equation}  \label{transversal}
        G_\Sigma+L=W
        \end{equation} 
        Define 
        $$W_k=\{ J\in W\mid J_n=0,n\geq k\}$$
        so $H=W_1\subset W_2\subset...\subset W_k\subset W_{k+1}\subset ... \subset W=\cup_{k>0} W_k$.  We have $\dim(W_k/W_{k-1})=|R|$ and by Riemann-Roch this vector space can be represented by elements of $G_\Sigma$ since
        \begin{align*}
        \dim(W_k\cap G_\Sigma)-\dim(W_{k-1}\cap G_\Sigma)&=\dim H^0(K(kR))-\dim H^0(K((k-1)R))\\
        &=k|R|+1-g-((k-1)|R|+1-g)=|R|.
        \end{align*}
        Hence $\left(W_k\cap G_\Sigma\right)+L=W_k$ and 
        \eqref{transversal} follows by taking the union over $k>0$.
        
        Define $V_\Sigma \subset G_\Sigma$ to consist of those differentials with vanishing $\ca$-periods.  It is easy to see that the proof of \eqref{transversal} can be adjusted to yield:
        $$ V_\Sigma \oplus L= W
        $$
        since the elements of $W_k\cap G_\Sigma$ can be chosen to be normalised to have vanishing $\ca$-periods.
        
        Let $\eta_1+\ell\in G_\Sigma^\perp$ for $\eta_1\in V$ and $\ell\in L$.  Then $\omega(\eta_1+\ell,\eta_2)=0$ for all $\eta_2\in V$ since $ \eta_1+\ell$ annihilates all elements of $G_\Sigma$, in particular those from $V$.  But $\omega(\eta_1,\eta_2)=0$ by the Riemann bilinear relations:
        \begin{equation}  \label{RiemBilRel}
        \sum\Res_{r\in R} f_1\eta_2=\frac{1}{2\pi i}\sum_{k=1}^g\oint_{b_j}\eta_1\oint_{a_j}\eta_2-\oint_{b_j}\eta_2\oint_{a_j}\eta_1=\frac{1}{2\pi i}\int_\Sigma[\eta_1]\wedge[\eta_2]
        \end{equation}
        since all $\ca$-periods vanish in the middle expression of \eqref{RiemBilRel}.  Here $df_1=\eta_1$ for a locally defined function $f_1$.  Hence $\omega(\ell,\eta_2)=0$ for all $\eta_2\in V$.  But $\omega$ is symplectic, so for any non-zero $\ell\in L$ there is $\eta_2\in V$ such that $\omega(\ell,\eta_2)\neq 0$.  We conclude that $\ell=0$ so $\eta_1+\ell=\eta_1\in V$, hence 
        $$G_\Sigma^\perp\subset V\subset G_\Sigma$$
        as required.
        \end{proof}
        We can strengthen Lemma~\ref{coisotropic} to get exactness of elements in $G_\Sigma^{\perp}$, i.e.
        $$
        G_\Sigma^{\perp}=\{ \eta=df,\  f \text{\ holomorphic on }\Sigma-R\}
        $$
        as follows.  The inclusion of exact differentials into $G_\Sigma^{\perp}$ follows
        from the fact that if $\eta_1=df_1$ for a {\em global} meromorphic function $f_1$ then $\sum\Res_{r\in R} f_1\eta_2=0$ since it is the sum of the residues of the meromorphic differential $f_1\eta_2$.  For the other direction, by Lemma~\ref{coisotropic}, any $\eta_1\in G_\Sigma^{\perp}$ lives in $G_\Sigma$ hence it is (the local expansion of) a globally defined meromorphic differential on $\Sigma$.  The $\cb$-periods of $\eta_1$ can be calculated using \eqref{RiemBilRel}.  Let $\omega_i$, $i=1,...,g$ be the normalised holomorphic differentials on $\Sigma$, so $\oint_{a_j}\omega_i=\delta_{ij}$.  We have
        $$
        \oint_{b_j}\eta_1=\oint_{a_j}\omega_j\oint_{b_j}\eta_1-\oint_{a_j}\eta_1\oint_{b_j}\omega_j=\omega(\eta_1,\omega_j)=0
        $$
        since $\omega_j\in G_\Sigma$ and $\eta_1\in G_\Sigma^{\perp}$.  But the residues of $\eta_1$ and all of its $\ca$-periods and $\cb$-periods vanish.  Hence 
        $$f(p):=\int^p_{p_0}\eta_1$$
        is well-defined and $\eta_1$ is exact.
        
        Thus the symplectic quotient of $W$ is given by
        $$ W\sslash G_\Sigma^\perp:=G_\Sigma/G_\Sigma^\perp\cong H^1(\Sigma,\bc)
        $$
        where the last equality uses the fact that elements of $G_\Sigma$ define cohomology classes on $\Sigma$, the quotient by exact differentials sends a meromorphic differential (with zero residues) to its cohomology class, and the map is surjective.  Clearly
$$V_\Sigma\to\overline{V}_\Sigma=V_\Sigma/G_\Sigma^\perp$$
where $\overline{V}_\Sigma\subset H^1(\Sigma;\bc)$ consists of those cohomology classes with vanishing $A$-periods.
        
        %\begin{itemize}
        
        %\item $\bw\stackrel{Lag.}{\supset} L=\{$loc. holo$^c$ diff$^\ell\}\mapsto H^0(K_\Sigma)\stackrel{Lag.}{\subset} H^1(\Sigma,\bc)$
        %\end{itemize}
\subsection{The quadratic Lagrangian \texorpdfstring{$\cl$}{L}.}        
Given a symplectic quotient
$$ M\sslash G:=\mu^{-1}(a)/G$$
and a Lagrangian submanifold $\cl\subset M$, if $\cl$ intersects $\mu^{-1}(a)$ transversally, then the quotient of $\cl\cap\mu^{-1}(a)$ defines a Lagrangian submanifold of $\mu^{-1}(a)/G$.  The intersection $\cl\cap G_\Sigma$ is transversal by \eqref{transversal} since $T_0\cl=L$   

To make sense of the quotient of $\cl\cap G_\Sigma$, since $\cl$ lives in a formal neighbourhood of $0\in W$, we need to treat symplectic reduction of $(W,\Omega_W)$ algebraically.
The quotient
$$G_\Sigma^\perp\to G_\Sigma\to H^1(\Sigma;\bc)
$$
corresponds to the ring homomorphism
\begin{align*}
k[H^1(\Sigma;\bc)]&\to k[G_\Sigma]^{G_\Sigma^\perp}\\
(z^i,\w_i)&\mapsto(\oint_{a_i},\oint_{b_i})
\end{align*}
where $k[V]=\bigoplus_kSym^k(V^*)$ is the ring of regular functions on the vector space $V$.
Then
$$\cl\cap G_\Sigma\to \cb\subset G_\Sigma/G_\Sigma^\perp
$$
corresponds to
\begin{align*}
k[\cb]&\to k[\cl]\\
k \llbracket z^1,...,z^g \rrbracket &\to k \llbracket x^1,...,x^g \rrbracket.
\end{align*}
%do we need to prove that the image is $\cb$? it should follow form $\theta$ 

For $L=T_0\cl\subset W$ given by the Lagrangian subspace of locally holomorphic differentials, defined in a neighbourhood of $R\subset\Sigma$, the symplectic form $\Omega_W$ defines a natural isomorphism of Lagrangian subspaces $L\cong V_\Sigma^*$.  In the symplectic quotient $H^1(\Sigma;\bc)$, the symplectic form $\Omega$ defines a natural isomorphism of Lagrangian subspaces $H^0(K_\Sigma)\cong \overline{V}_\Sigma^*$.  These natural isomorphisms produce the following commutative diagram.
$$
\begin{tikzcd}
V_\Sigma\otimes V_\Sigma\otimes V_\Sigma\arrow{d}\arrow{r}{\Omega_W}  &\text{Hom}(L\otimes L,V_\Sigma)\arrow{d}  \\
\overline{V}_\Sigma\otimes \overline{V}_\Sigma\otimes \overline{V}_\Sigma  \arrow{r}{\Omega} &
\text{Hom}(H^0(K_\Sigma)\otimes H^0(K_\Sigma),\overline{V}_\Sigma) \end{tikzcd}
%\quad\mathrel{\mathop{\longrightarrow}^{\cong}_{\Omega_W}}\quad
$$
The right vertical arrow is induced from the map 
$$h:H^0(K_\Sigma)\to L$$
which maps a holomorphic differential to its local expansion at $R\subset\Sigma$.  Hence
$$
 \begin{tikzcd} L\otimes L\arrow{r}{T} & V_\Sigma \arrow{d} \\ H^0(K_\Sigma)\otimes H^0(K_\Sigma)\arrow{r} \arrow{u}{h\otimes h} & \overline{V}_\Sigma  \end{tikzcd} 
$$
and $T\mapsto[T\circ (h\otimes h)]$
%$T\mapsto[T(h(\eta_1)\otimes h(\eta_2))]\in \text{Hom}(H^0(K_\Sigma)\otimes H^0(K_\Sigma),\overline{V}_\Sigma)$
where $[\cdot]$ is the map $V_\Sigma\to\overline{V}_\Sigma$.
    
    \subsection{Quantum Airy structures}
    
    Now let \( \mathcal{W} = \mathbf{k}\llbracket x^{\sbt}, \hbar \partial_{\sbt} \rrbracket \llbracket \hbar \rrbracket \) be a graded Weyl algebra with Lie bracket given by \( [ x_i , x_i] =  [\partial_i, \partial_j ] = 0\) and \( [\hbar \partial_i , x^j ] =  \delta^j_i \).

    Consider the differential operators \(\widehat{H}'_i \in \mathcal{W} \) 
    \begin{align*}
            \widehat{H}'_i = \hbar \partial_i + a_{ijk} x^i x^j +   2 \hbar \,  b_{ij}^k  \, x^j \partial_k + \hbar^2 c_{i}^{jk} \partial_j \partial_k.
    \end{align*}
        
    %\begin{defn}[pre-quantum Airy structure] 
    %A \emph{pre-quantum Airy structure} is a choice of coefficients \( (a_{ij}^k,b_{ij}^k,c_{i}^{jk})\), such that the \(\widehat{H}_i\) are closed under the Lie bracket \( [\widehat{H}_i , \widehat{H}_j] = g_{ij}^k \widehat{H}_k\). This gives the same constraints as the Airy structure.
    %\end{defn}

    Kontsevich and Soibleman define a \emph{quantum Airy structure} as the deformation quantisation of the classical Airy structure on the formal Lagrangian. Deformation quantisation is a functor which replaces the commutative algebra \( \mathbf{k}\llbracket x^{\sbt}, y_{\sbt} \rrbracket \) with the non commutative Weyl algebra of differential operators \( \mathcal{W} \). First the coordinates are mapped by \( x_i \rightarrow x_i \) and \( y_i \rightarrow \hbar \partial_i \). \(\partial_i \) can be identified with the vector field, or derivation, \( \frac{\partial}{\partial x^i}\) when \( \hbar \) is invertible.  
    
    Further the Poisson Lie algebra \( \mathfrak{g}\) with Poisson bracket has to be identified with the Lie algebra structure of the \(\widehat{H}_i\) with a Lie bracket. A necessary condition to do this, is that the second cohomology vanishes, \(H^2(\mathfrak{g}, \mathbf{k})=0\). This is a choice of central extension to \(\mathfrak{g}\) so the Lie algebra structure of the quantum and classical cases coincide. So  
    \[ H_i \rightarrow \widehat{H}_i = \widehat{H}'_i + \hbar \varepsilon_i,\] 
    and 
    \[ [\widehat{H}_i, \widehat{H}_j] = \hbar \{ H_i , H_j \}_{x^{\sbt}\rightarrow x^{\sbt}, y_{\sbt} \rightarrow \hbar \partial_{\sbt}} + \hbar g_{ij}^k \varepsilon_k.\]
    
    \begin{defn}[quantum Airy structure]
    A \emph{quantum Airy structure} is the collection of \( \widehat{H}_i := \widehat{H}_i + \hbar \varepsilon_i\), and an extra constraint:
    \[ 2 \left( a_{jst} \, c_i^{st} - a_{ist} \, c_j^{st} \right) = g_{ij}^k \varepsilon_k.\]
    \end{defn}
    
    When a quantum Airy structure arises from deformation quantisation, this gives rise to a wavefunction supported on \(\mathcal{L}\). A wavefunction is a generator of a cyclic module \(\mathcal{D}\) over \(\mathcal{W}\), given by the quotient \( \mathcal{D} = \mathcal{W} / \mathcal{W} \langle \widehat{H}_i \rangle  \). This module encodes the solution to the \(\widehat{H}_i\) acting as operators on \( \mathbf{k}\llbracket x^{\sbt} \rrbracket \llbracket \hbar \rrbracket \). The wavefunction \( \psi_{\mathcal{L}} \in \mathbf{k}\llbracket x^{\sbt} \rrbracket \llbracket \hbar \rrbracket\) can be computed using the ansatz 
    \[ \psi_{\mathcal{L}} = \exp(S(x^{\sbt})),\]
    where
    \[ S(x^{\sbt}) = \sum_g \hbar^{g-1} S_g(x^{\sbt}),\]
    and solving the differential equations
    \[ \widehat{H}_i \exp(S(x^{\sbt})) = 0. \] 
    Modulo \(\hbar \) this is a function supported on \( \widehat{\mathcal{L}}\).
    Individually \(S_g(x^{\sbt}) \in \mathbf{k} \llbracket x^{\sbt}\rrbracket\). \

    \begin{example} Consider the quantised conic with \( \varepsilon = 0\):
    \[ \left( - \hbar \frac{\partial}{\partial x} + x^2 + 2 \hbar x \frac{ \partial }{\partial x}+ \hbar^2 \frac{\partial^2}{\partial^2 x} \right) \psi_{\mathcal{L}}(x) = 0. \]
    Computing some terms
    \[ \psi_{\mathcal{L}}(x) = \exp \left( \frac{1}{\hbar} \int dx \, ( u_0(x)  + \hbar \, u_1(x) + \mathcal{O}(\hbar^2) ) \right), \]
    with \( u_0(x)\) as before, and \(u_1(x) = 2 x + 10 x^2 + \cdots + (4^n - \frac{(2n)!}{(n!)^2}) x^n + \cdots \) a generating function for counting numbers of rooted two-face \(n\)-edge maps in the plane, (1-loop Feynmann diagrams) \cite{feynmaps}.
    \end{example}

    A significant result of Kontsevich and Soibelman is that the coefficients of \(S_{g,n}\) of \(S\) satisfy \emph{abstract topological recursion}.  
    
    Eynard Orantin topological recursion \cite{eynard_orantin}, can be seen as a particular specialisation of abstract topological recursion. Restricting to the odd \(H_i\) recovers topological recursion. The identification with the tensors in \(\widehat{\mathrm{Sym}}(V)\) proves the symmetry of \( \omega_{g,n}\).    
    
    \subsection{Formal geometry of Airy structures}
\label{formal}



Consider a symplectic surface $(X,\omega)$ with a Lagrangian foliation $\cF$. 

Let \(p \in X\). A formal disc \(\mathbb{D}\) is an infinitesimal neighbourhood of \(p\). Let  \( \pi : \mathbb{D} \rightarrow p\) be an embedding of a formal disc into \(X\). 

% eg C[t]/t^2 ~= Disc^(1) ?

Let $Discs^{(n)}$ be the space of $n$-jets of embedded formal discs in $X$ which are tangent to a leaf of the foliation with the tangency order one.

%A disc is a local artin algebra \( Discs^{(n)} \simeq \mathbb{C}[z]/z^n dz\).

The space of formal discs, \( Discs\) is the projective limit 
%of the projective system of fibrations 
\[ Discs = \lim_n Discs^{(n)}\]
understood in the category of local Artin algebras.

Any point $t \in Discs$ defines the corresponding formal disc embedded in the surface $X$ denoted by $\widehat{\bd}_t$.
For any such point $t$ the tangent space $T_t Discs$ is isomorphic with the cotangent space of $\widehat{\bd}_t$ which can be identified with the infinite dimensional vector space $\bc \llbracket z\rrbracket dz$.
Denote by $UnivDiscs$ (resp $UnivDiscs^*$) the total space of the fibration over $Discs$ with fiber $\widehat{\bd}_t$, (resp $\widehat{\bd}_t^*$) at the point $t \in Discs$. There is a canonical non-linear flat connection $\nabla_{univ}$ on the fibration $UnivDiscs^* \rightarrow Discs$ which is defined using the foliation $\cF$.

Consider symplectic vector bundle \( \ch\) with fibers consisting of vector spaces 

$$\ch_t=\{\gamma \in \Omega^1( \hat{\bd}_t^*): \mathrm{Res}(\gamma)=0\}.$$

The formal version of Theorem \ref{Lagrangian} is the following:

\begin{theorem}[Kontsevich-Soibelman]
For a given foliated symplectic surface $X$ and a spectral curve $\Sigma$ there is a flat section $\phi$ of the flat connection $\nabla_{univ}$ corresponding to 

$$T_t Discs =\Omega^1(\hat{\bd}_t) \rightarrow \mathrm{Ker} \left( \mathrm{Res}: \Omega^1(\hat{\bd}_t^*) \rightarrow \bc \right) = \ch_t$$
defines a Lagrangian embedding of the tangent bundle $T_{Discs}$ into the symplectic bundle $\ch$.
\end{theorem}



    
    
\subsection{Quantum Airy structure from Higgs bundles}

Recall, the base of the Hitchin system can be identified with the moduli space of deformations of $\Sigma$ inside the symplectic surface $T^* C$. 
Let $\Sigma \rightarrow C$ be a simple ramified covering, with ramification points \(Ram\). Note that there are $|Ram|=2n(n-1)(g-1)$ ramification points. As shown previously, there exists a symplectic vector space $W= \otimes_{r \in Ram} W_{Airy}$.

As we have seen in Section \ref{section:universal} the vector space $W$ can be decomposed as the direct sum $V \oplus V^*$, with a corresponding Airy structure.

Furthermore, this Airy structure can be quantised via deformation quantisation, shown by \cite{KSoAir}, and described in the previous section \ref{}. This quantisation gives a wave function of the form 
$$\psi_{\mathcal{L}}=\exp \left(S_0/\hb+\sum_{g \geq 1} S_g \hb^{g-1} \right).$$

The resulting quantum Airy structure captures useful information about the special K\"ahler geometry of the moduli space $\cb^{reg}$.
A prepotential for the special K\"ahler geometry is given by $F=\frac{1}{2} \sum_i z^i w_i$. The period matrix is given by $\tau_{ij}=\frac{\partial w_i}{\partial z^j}$, which is the same as $\frac{\partial^2 F}{\partial z^i \partial z^j}$.

    Recall that the Donagi-Markman cubic is given by
    $$c=\sum_{i,j,k} c_{ijk} dz^i \otimes dz^j \otimes dz^k,$$
    where 
    \[c_{ijk}=\frac{\partial \tau_{jk}}{\partial z^i}=\frac{\partial^3 F}{\partial z^i \partial z^j \partial z^k}.\]
    The connection between the Donagi-Markman cubic and the prepotential is studied in \cite{BHuSpe}. Using a version of Rauch variation formula it is proved that
    $$c_{ijk}=-\left(\frac{i}{2\pi}\right)^2 \int_{p \in b_i} \int_{p_1 \in b_j} \int_{p_2 \in b_k} \omega_{0,3}(p,p_1,p_2).$$
    In the Airy structure picture, the prepotential corresponds to the genus zero part of the wavefunction \( \psi_{\mathcal{L}}\).


\begin{proposition}
    Let $n,d$ be natural numbers. Consider the moduli space of Higgs bundles of rank $n$ and degree $d$ on a compact Riemann surface $C$ of genus $g>1$, together with the Hitchin system $f:\cm \to \cb$. For any point $b \in \cb^{reg}$ consider the associated Quantum Airy structure and the resulting wave function $\psi_{\mathcal{L}}$. Then
    $$\partial_{i_1} \partial_{i_2} \dots \partial _{i_{m-2}} \tau_{i_{m-1} i_m}(b)=-\left(\frac{i}{2\pi}\right)^{m-1} \int_{p_1 \in b_{i_1}} \dots \int_{p_m \in b_{i_m}} \omega_{0,m}(p_1,\dots,p_m),$$
    where $\omega_{0,m}$ are Eynard-Orantin invariants of the spectral curve $S_b$.
    \end{proposition}
    \begin{proof}
    This follows immediately from Theorem 1.
    \end{proof}


    In \cite[Theorem 1.3]{BHuSpe} it is also proved that for any point $b \in \cb^{reg}$,  they have the same relationship between the Taylor expansion of the prepotential and $B$-periods of the genus zero component $S_0$ of the wave function (although they used a different language). 
    
    It is mentioned that this formula is remarkable since the left hand side is related to geometry of a family of curves, while the right hand side only involves invariants of a single spectral curve. The results proved in this article show that this phenomenon occurs more generally. The same result occurs when the moduli space $\cb$ does not necessarily come from Higgs bundles. 

    
    % existence of 

    
    
    % ideal <H_i>
    % completion k[x1,..y1,..] -> k\llbracketx1,....y1..\rrbracket
    % ind scheme scheme
    % defines curly L at a point
     
    
    % S_0^{(n-1)

    
    % define map S_0^{(n-1)} \rightarrow S_0^{(n)} 
    
    
    
    
    % S_{0;i}^{(n)} = a_{ijk} x^j x^k + b_ij^k x^j S^{(n-1)}_{0;k} + c_{i}^{jk} S^{(n-1)}_{0;j} S^{(n-1)}_{0;k}
    
    
    % curly L associated Lie algebra
        
    % formal vector fields on curly L (Lie algebra automorphism)
    
    %A formal vector field on \( \mathcal{L} \) can be represented by a derivation on \( \mathbf{k}\llbracket x^{\sbt} \rrbracket\).
    
    % deformation of Lie algebra
    
    % on level of H_i can consider map H -> \hat{H}
    
    % sends S_0 -> S_g
    
    %briefely mention topological recursion / cite ks restriction of tensors gives TR.       

    % formal germ algorithm

    %topological recursion from airy structure

==> slhiggsbundle.tex <==
\section{Higgs Bundles With Other Gauge Groups} 
So far we have studied how the idea of Kontsevich-Soibelman can be used to study the deformations of spectral curves associate with $GL(n,\mathbb{C})$-Higgs bundles. In this section we will investigate the situation where $GL(n,\mathbb{C})$ is replaced by other classical groups, namely: $SL(n,\mathbb{C})$, $Sp(2n, \mathbb{C})$, $SO(2n, \mathbb{C})$ and $SO(2n+1, \mathbb{C})$. In general a $G$-Higgs bundle is given by a pair $(E,\Phi)$ where $E$ is a (semi)stable vector $G$-bundle over a curve $C$ and $\Phi \in \Gamma(C,P\otimes K_C)$ where $P$ is the principal $G$-bundle such that $E \cong P\times_G \mathbb{C}^n$. The Hitchin fibration is given by
\begin{equation*}
    h : \mathcal{M}_{n,d}^G \rightarrow \mathcal{B}^G := \bigoplus_{i=1}^k H^0(C, K^{d_i}), \qquad (E,\Phi) \mapsto (a_1(\Phi),\cdots,a_k(\Phi)),
\end{equation*}
where $a_i(\Phi)$ are $G$-invariant polynomials of degree $d_i$ given by
\begin{equation*}
    \det(\lambda - \Phi) =: \lambda^n + \sum_{i=1}^k \pi^*a_i(\Phi)\lambda^{n-d_i}.
\end{equation*}
Let $\Sigma_b \subset T*C$ be the spectral curve given by the zero divisor of $\det(\lambda - \Phi) \in H^0(T^*C, \pi^*K^n)$. Generically, $\Sigma_b$ is a genus $g = n^2(g_C-1) + 1$ smooth Riemann surface. We have seen that when $G = GL(n, \mathbb{C})$ the fiber $h^{-1}(b)$ over any point $b \in \mathcal{B}^{GL(n,\mathbb{C})}$ is isomorphic to $Jac(\Sigma_b)$. As we will see, this will not be the case for $G \neq GL(n,\mathbb{C})$, although it is always true that $\dim \mathcal{B}^G = \dim h^{-1}(b) = \frac{1}{2}\dim\mathcal{M}_{n,d}^G$.

\subsection{\texorpdfstring{$SL(n,\mathbb{C})$}{SL(n,C)}-Higgs Bundles}
In this case, we have that $tr(\Phi) = 0$ and therefore 
\begin{equation}\label{sigmabequation}
\det(\lambda - \Phi) = \lambda^n + \pi^*a_2(\Phi)\lambda^{n-2} + \cdots + \pi^*a_n(\Phi).
\end{equation}
It follows that $\mathcal{B}^{SL(n,\mathbb{C})} = \bigoplus_{i=2}^nH^0(C,K^i)$ and $\dim\mathcal{B}^{SL(n,\mathbb{C})} = (n^2-1)(g-1)$.
It has been shown (for example, see \cite{schaposnik2014introduction}) that $h^{-1}(b) = Prym(\Sigma_b,C)$. The \emph{Prym variety} $Prym(\Sigma_b,C)$ is given by
\begin{equation*}
    0\rightarrow Prym(\Sigma_b,C) \rightarrow Jac(\Sigma_b) \xrightarrow{Nm} Jac(C) \rightarrow 0
\end{equation*}
where $Nm : Pic(\Sigma_b) \rightarrow Pic(C)$ denotes the Norm map, let $\pi : \Sigma_b \rightarrow C$ be the canonical projection then $Nm(\sum_{i}n_ip_i) = \sum_in_i\pi(p_i)$. Taking the homology long exact sequence and the cap product duality between holomogies and cohomologies with field coefficients, we arrive at the following commutative diagram with exact rows:
\begin{equation*}
    \begin{tikzcd}
    0 \arrow{r} & H^1(Prym(\Sigma_b, C), \mathbb{C}) \arrow{r} \arrow{d}{\cong} & H^1(Jac(\Sigma_b), \mathbb{C}) \arrow{r}{Nm_!}\arrow{d}{\cong} & H^1(Jac(C), \mathbb{C}) \arrow{r}\arrow{d}{\cong} & 0\\
    0 \arrow{r} & H_1(Prym(\Sigma_b, C), \mathbb{C}) \arrow{r} & H_1(Jac(\Sigma_b), \mathbb{C}) \arrow{r}{Nm_*} & H_1(Jac(C), \mathbb{C}) \arrow{r} & 0    
    \end{tikzcd}
\end{equation*}
We also know that $H_1(Jac(\Sigma_b), \mathbb{C}) \cong H_1(\Sigma_b, \mathbb{C})$ and $H_1(Jac(C), \mathbb{C}) \cong H_1(C,\mathbb{C})$. Since it is always possible to choose $A$, $B$-cycles that do not intersect any ramification points of the cover $\pi: \Sigma_b \rightarrow C$, therefore given a symplectic basis $\{A_l, B_l\ |\ l = 1,\cdots,g_C\}$ there exists cycles $A^k_l, B^k_l \in H_1(\Sigma_b, \mathbb{C}), k = 1,\cdots,n$ such that $A_l = \pi(A^k_l)$ and $B_l = \pi(B^k_l)$. Hence, we can write a symplectic basis for $H_1(\Sigma_b, \mathbb{C})$ as 
\begin{equation*}
    \{A^1_l, B^1_l,\cdots, A^n_l, B^n_l, C_i, D_i\ |\ l = 1,\cdots,g_C, i = 1,\cdots,g - ng_C\},
\end{equation*}
where $g = n^2(g_C-1)+1$ is the genus of $\Sigma_b$. Let us denote the symplectic dual basis for $H^1(\Sigma_b, \mathbb{C}) \cong H_1(\Sigma_b, \mathbb{C})^*$ by 
\begin{equation*}
    \{\xi^1_l, \eta^1_l, \cdots, \xi^n_l, \eta^n_l, \epsilon_i, \delta_i\ |\ l = 1,\cdots,g_C, i = 1,\cdots, g-ng_C\}
\end{equation*}
where $\xi^k_l, \eta^k_l, \epsilon_i, \delta_i$ can be thought of meromorphic differentials on $\Sigma_b$ such that
\begin{equation*}
    \oint_{A_{l_1}^{k_1}}\xi^{k_2}_{l_2} = \oint_{B_{l_1}^{k_1}}\eta_{l_2}^{k_2} = \delta^{k_1k_2}\delta_{l_1l_2}, \qquad \oint_{C_i}\epsilon_j = \oint_{D_i}\delta_j = \delta_{ij},
\end{equation*}
and all other integrals vanish. Then it follows that $Nm_!(\xi^k_l) = \xi_l, Nm_!(\eta^k_l) = \eta_l, Nm_!(\epsilon_i) = Nm_!(\delta_i) = 0$ where $\{\xi_l, \eta_l\}$ is a basis of $H^1(C,\mathbb{C})$ satisfying $\oint_{A_i}\xi_j = \oint_{B_i}\eta_j = \delta_{ij}, \oint_{A_i}\eta_j = \oint_{B_i}\xi_j = 0$. Now that we have established the necessary notations, the following expression for $H^1(Prym(\Sigma_b, C), \mathbb{C}) = \ker Nm_!$ is clear:
\begin{lemma}
    \begin{equation*}
    H^1(Prym(\Sigma_b, C), \mathbb{C}) \cong \left\{\xi \in H^1(\Sigma_b, \mathbb{C})\ |\ \sum_{k=1}^n\oint_{A_l^k}\xi = \sum_{k=1}^n\oint_{B_l^k}\xi = 0, l = 1,\cdots,g_C\right\}.
    \end{equation*}
\end{lemma}
\begin{proof}
First, let us recall that $H^1(Prym(\Sigma_b, C),\mathbb{C}) \cong \ker Nm_!$. In general, any $\xi \in H^1(\Sigma_b, \mathbb{C})$ can be written as $\xi = \sum_{l=1}^{g_C}\sum_{k=1}^n\left(\left(\oint_{A^k_l}\xi\right)\xi^k_l + \left(\oint_{B^k_l}\xi\right)\eta^k_l\right) + \sum_{i=1}^{g-ng_C}\left(\left(\oint_{C_i}\xi\right)\epsilon_i + \left(\oint_{D_i}\xi\right)\delta_i\right)$. Then 
\begin{align*}
    \xi \in \ker Nm_! &\iff Nm_!\xi = \sum_{l=1}^{g_C}\left(\left(\sum_{k=1}^n\oint_{A^k_l}\xi\right)\xi_l + \left(\sum_{k=1}^n\oint_{B^k_l}\xi\right)\eta_l\right) = 0\\
    &\iff \sum_{k=1}^n\oint_{A^k_l}\xi = \sum_{k=1}^n\oint_{B^k_l}\xi = 0, l = 1,\cdots, g_C.
\end{align*}
\end{proof}

Previously, we have defined the coisotropic subspace $G_\Sigma \subset W^{Ram}_{Airy}$ such that $G_\Sigma/G^\perp_\Sigma \cong \mathcal{H}_\Sigma$, and the Lagrangian complement $V_\Sigma$ given by meromorphism differentials with vanishing $A$-periods. In the case where $G=SL(n,\mathbb{C})$ we can modify the definition of each spaces as follows
\begin{align*}
    G_{\Sigma}^{SL(n,\mathbb{C})} &:= \left\{\xi \in G_\Sigma\ |\ \sum_{k=1}^n\oint_{A^k_l}\xi = 0, l = 1,\cdots,g_C\right\}\\
    V_{\Sigma}^{SL(n,\mathbb{C})} &:= V_{\Sigma}\\
    \left(G^{SL(n,\mathbb{C})}_{\Sigma}\right)^\perp &:= \left\{\xi \in G_\Sigma\ |\ \oint_{B^1_l}\xi = \cdots = \oint_{B^n_l}\xi, \oint_{A^k_l}\xi = \oint_{C_i}\xi = \oint_{D_i}\xi = 0\right\}.
\end{align*}
Note that we have $G^{SL(n,\mathbb{C})}_\Sigma/\left(G^{SL(n,\mathbb{C})}_{\Sigma}\right)^\perp \cong \left(H_1(Prym(\Sigma, C), \mathbb{C})\right)^* \cong H^1(Prym(\Sigma,C),\mathbb{C})$. The important point is that, although a class $[\xi] \in G^{SL(n,\mathbb{C})}_\Sigma/\left(G^{SL(n,\mathbb{C})}_{\Sigma}\right)^\perp$ is not a well-defined linear functional on $H_1(\Sigma, \mathbb{C})$ due to the ambiguity of adding $\xi' \in \left(G^{SL(n,\mathbb{C})}_{\Sigma}\right)^\perp$ such that $\oint_{B^1_l}\xi' = \cdots = \oint_{B^n_l}\xi' \neq 0$, it is a well-defined linear functional on $H_1(Prym(\Sigma, C),\mathbb{C})$. It is useful to define
\begin{equation*}
    \tilde{G}^{SL(n,\mathbb{C})}_\Sigma = \left\{\xi \in G_\Sigma\ |\ \sum_{k=1}^n\oint_{A^k_l}\xi = \sum_{k=1}^n\oint_{B^k_l}\xi = 0, l = 1,\cdots,g_C\right\}.
\end{equation*}
Then we have $G^{SL(n,\mathbb{C})}_{\Sigma} = \tilde{G}^{SL(n,\mathbb{C})}_{\Sigma} + \left(G^{SL(n,\mathbb{C})}_{\Sigma}\right)^\perp$ and $H^1(Prym(\Sigma,C), \mathbb{C}) \cong \tilde{G}^{SL(n,\mathbb{C})}_\Sigma/G^\perp_\Sigma$.

Let $[\Sigma_0] \in \mathcal{B}^{SL(n,\mathbb{C})}$ be fixed and let us define the map $\Phi^{SL(n,\mathbb{C})} := \Phi_{\Sigma_0}|_{\mathcal{B}^{SL(n,\mathbb{C})}} : \mathcal{B}^{SL(n, \mathbb{C})} \rightarrow G_{\Sigma_0}$ as we have done previously: $\Phi_{\Sigma_0}(\Sigma) := \theta_{\Sigma_0} - s^*_{\Sigma_0,\Sigma}\theta_{\Sigma}$.
\begin{lemma}\label{phislisintildeglemma}
    The image of $\Phi_{\Sigma_0}^{SL(n,\mathbb{C})}$ is contained inside $\tilde{G}^{SL(n,\mathbb{C})}_{\Sigma_0} \subset G_{\Sigma_0}$, in other words, we have the map $\Phi^{SL(n,\mathbb{C})}_{\Sigma_0} : \mathcal{B}^{SL(n,\mathbb{C})} \rightarrow \tilde{G}^{SL(n,\mathbb{C})}_{\Sigma_0}$.
\end{lemma}
\begin{proof}
Let $U$ be an open subset on the Riemann surface $C$ with local coordinates $q$, then $T^*U$ is an open subset of $T^*C$ with local coordinates $(q,p)$. We can write $\lambda$ locally as $\lambda|_{T^*U} = pdq$ and $\theta_{\Sigma}|_{T^*U\cap \Sigma} := (\lambda|_{T^*U})|_{\Sigma} = pdq|_{\Sigma}$. Suppose also that $\pi^*a_i(\Phi)|_{T^*U} = a_i(q;\Phi)(dq)^i \in H^0(T^*U, \pi^*K^i)$. Therefore, on the local coordinates chart $(T^*U,q,p)$, Equation (\ref{sigmabequation}) can be written as 
\begin{equation*}
    \left(p^n + a_2(q;\Phi)p^{n-2} + \cdots + a_n(q;\Phi)\right)(dq)^n = 0.
\end{equation*}
This means if $\{p_1,\cdots,p_n\} = \pi^{-1}(q)\cap \Sigma$ then $p_1 + \cdots + p_n = 0$, consequently: $\sum_{x \in \pi^{-1}(q)\cap \Sigma}\theta_x = (p_1+\cdots+p_n)dq = 0$. Now, let us consider $\{A^1_l, \cdots, A^n_l\}$ for some $l = 1,\cdots,g_C$ such that $\pi(A^k_l) = A_l$. Let us cover $A_l \subset C$ by a finite number of coordinates charts $(U_i, p_i, q_i), i = 1,\cdots, N$ and dissecting $A_l$ into $N$ disjoint segments $A_l = \coprod_{i=1}^N A_{l,i}$ such that $A_{l,i} \in U_i$. Then for each $k = 1,\cdots,n$, we have $A^k_l = \coprod_{i=1}^N A^k_{l, i}$ such that $A^k_{l,i} \subset U_i^k$ where $\pi^{-1}(U_i) = \Sigma\cap T^*U_i =: \coprod_{k=1}^nU^k_i$ and $\pi(A^k_{l,i}) = A_{l,i}$. Note that $q_i$ is a local coordinate on $U^k_i$ for every $k = 1,\cdots,n$ and $\theta|_{U^k_i} = p_{k,i}(q_i)dq_i$ where $\{p_{1,i}(q_i),\cdots,p_{n,i}(q_i)\} = \pi^{-1}(q_i)\cap \Sigma$. Therefore,
\begin{equation*}
    \sum_{k=1}^n\oint_{A^k_l}\theta_\Sigma = \sum_{k=1}^n\sum_{i=1}^N\int_{A^k_{l,i}}\theta_\Sigma = \sum_{i=1}^N\int_{A_{l,i}}\sum_{k=1}^np_{k,i}(q_i)dq_i = \sum_{i=1}^N\int_{A_{l,i}}0 = 0.
\end{equation*}
Similarly, it can be checked that $\sum_{k=1}^n\oint_{B^k_l}\theta = 0$. Since $\oint_{A^k_l \subset \Sigma_0}s^*_{\Sigma_0, \Sigma}\theta_{\Sigma} = \oint_{A^k_l \subset \Sigma}\theta_{\Sigma}$ and $\oint_{B^k_l \subset \Sigma_0}s^*_{\Sigma_0, \Sigma}\theta_{\Sigma} = \oint_{B^k_l \subset \Sigma}\theta_{\Sigma}$, it follows that
\begin{equation*}
\sum_{k=1}^n\oint_{A^k_l}\Phi_{\Sigma_0}(\Sigma) = \sum_{k=1}^n\oint_{B^k_l}\Phi_{\Sigma_0}(\Sigma) = 0    
\end{equation*}
proving the lemma.
\end{proof}

\begin{corollary}
The image of $[\Phi^{SL(n,\mathbb{C})}_{\Sigma_0}]$ is contained inside $H^1(Prym(\Sigma_0, C),\mathbb{C}) \subset \mathcal{H}_{\Sigma_0}$, in other words, we have the map $[\Phi^{SL(n,\mathbb{C})}_{\Sigma_0}] : \mathcal{B}^{SL(n,\mathbb{C})}\rightarrow H^1(Prym(\Sigma_0,C),\mathbb{C})$.
\end{corollary}

Now, let us choose a more convenient symplectic basis of $H^1(\Sigma,\mathbb{C})$ for working with with subspace $H^1(Prym(\Sigma, C),\mathbb{C})$ as follows:
\begin{equation*}
    \{\tilde{\xi}^1_l, \tilde{\eta}^1_l, \cdots, \tilde{\xi}^n_l, \tilde{\eta}^n_l, \epsilon_i, \delta_i\ |\ l = 1,\cdots,g_C, i = 1,\cdots, g-ng_C\}
\end{equation*}
where
\begin{align*}
    \tilde{\xi}^k_l = T^k_l(\{\xi^{k'}_{l'}\}) &:= \begin{cases}
    \xi^{k}_l - \xi^{k+1}_l, & k = 1,\cdots,n-1\\
    \xi^1_l + \cdots + \xi^n_l, & k = n
    \end{cases}, \\
    \tilde{\eta}^k_l = ((T^{-1})^T)^k_l(\{\eta^{k'}_{l'}\})  &:= \begin{cases}
    \frac{n-k}{n}\sum_{i=1}^k\eta^i_l - \frac{k}{n}\sum_{i=k+1}^n\eta^i_l, & k = 1,\cdots,n-1\\
    \frac{1}{n}(\eta^1_l + \cdots + \eta^n_l), & k = n.
    \end{cases}
\end{align*}
Clearly, the subspace $H^1(Prym(\Sigma,C),\mathbb{C}) \subset H^1(\Sigma,\mathbb{C})$ is spanned by $\{\tilde{\xi}^1_l,\tilde{\eta}^1_l,\cdots,\tilde{\xi}^{n-1}_l, \tilde{\eta}^{n-1}_l,\epsilon_i,\delta_i\}$. The restriction of the symplectic form $\Omega_{\mathcal{H}}$ gives $H^1(Prym(\Sigma,C),\mathbb{C})$ the structure of symplectic vector space. Let us choose the corresponding symplectic basis for $H_1(\Sigma,\mathbb{C})$ as follows:
\begin{equation*}
    \{\tilde{A}^1_l,\tilde{B}^1_l, \cdots, \tilde{A}^n_l, \tilde{B}^n_l, C_i, D_i\ |\ l = 1,\cdots,g_C, i = 1,\cdots, g-ng_C\}
\end{equation*}
where $\tilde{A}^k_l := ((T^{-1})^T)^k_l(\{A^{k'}_{l'}\}), \tilde{B}^k_l := T^k_l(\{B^{k'}_{l'}\})$ and the subspace $H_1(Prym(\Sigma,C),\mathbb{C})$ is spanned by $\{\tilde{A}^1_l,\tilde{B}^1_l,\cdots,\tilde{A}^{n-1}_l, \tilde{B}^{n-1}_l, C_i, D_i\}$. Then, given $\xi_1,\xi_2 \in H^1(Prym(\Sigma,C),\mathbb{C})$, their symplectic pairing is given by
\begin{equation*}
    \Omega_{\mathcal{H}}(\xi_1,\xi_2) = \frac{1}{2\pi i}\sum_{l=1}^{g_C}\sum_{k=1}^{n-1}\left(\oint_{\tilde{A}^k_l}\xi_1\oint_{\tilde{B}^k_l}\xi_2 - \oint_{\tilde{A}^k_l}\xi_2\oint_{\tilde{B}^k_l}\xi_1\right) + \frac{1}{2\pi i}\sum_{i=1}^{g-ng_C}\left(\oint_{C_i}\xi_1\oint_{D_i}\xi_2 - \oint_{C_i}\xi_2\oint_{D_i}\xi_1\right).
\end{equation*}
Let us define
\begin{equation*}
    \tilde{a}^k_l(\Sigma) := \oint_{\tilde{A}^k_l}\theta_\Sigma, \qquad a_i(\Sigma) := \oint_{C_i}\theta_\Sigma, \qquad \tilde{b}^k_l(\Sigma) := \oint_{\tilde{B}^k_i}\theta_\Sigma, \qquad b_i(\Sigma) := \oint_{D_i}\theta_\Sigma.
\end{equation*}
Using $\{\tilde{a}^k_l, a_i\}$ as a coordinates system for $\mathcal{B}$ then $\mathcal{B}^{SL(n,\mathbb{C})} = \{\tilde{a}^n_1 = \cdots = \tilde{a}^n_{g_C} = 0\} \subset \mathcal{B}$. In the following, let $v^k_l := \frac{\partial}{\partial a^k_l}$ and $\tilde{v}^k_l := \frac{\partial}{\partial \tilde{a}^k_l}$. Since $\tilde{v}^k_l = v^k_l - v^{k+1}_l \in T_{\Sigma}\mathcal{B}^{SL(n,\mathbb{C})} \subset T_\Sigma \mathcal{B}$ and we know from Lemma \ref{phislisintildeglemma} that $\Phi_{\Sigma_0}(\Sigma) \in \tilde{G}^{SL(n,\mathbb{C})}_{\Sigma_0}$ for all $[\Sigma] \in \mathcal{B}^{SL(n,\mathbb{C})}$, therefore 
\begin{equation*}
    \sum_{k'=1}^n\oint_{A^{k'}_{l'}}\iota_{\tilde{v}^k_l}\nabla_{\mathcal{F}}\Phi_{\Sigma_0}(\Sigma) = \frac{\partial}{\partial\tilde{a}^k_l}\sum_{k'=1}^n\oint_{A^{k'}_{l'}}\Phi_{\Sigma_0}(\Sigma) = \frac{\partial}{\partial \tilde{a}^k_l}\left(\substack{\text{constant (= 0)}\\ \text{in $\tilde{a}^k_l$}}\right) = 0.
\end{equation*}
Similarly, $\sum_{k'=1}^n\oint_{B^{k'}_{l'}}\iota_{\tilde{v}^k_l}\nabla_{\mathcal{F}}\Phi_{\Sigma_0}(\Sigma) = 0$. This implies that $\iota_{\tilde{v}^k_l}\nabla_{\mathcal{F}}\Phi_{\Sigma_0}(\Sigma) \in \tilde{G}^{SL(n,\mathbb{C})}_{\Sigma_0}$. On the other hand, we have that $\Omega_{\mathcal{H}}(\iota_{\tilde{v}^{k_1}_{l_1}}\nabla_{\mathcal{F}}\Phi_{\Sigma_0}, \iota_{\tilde{v}^{k_2}_{l_2}}\nabla_{\mathcal{F}}\Phi_{\Sigma_0}) = 0$. Or, equivalently $\frac{\partial\tilde{b}^{k_2}_{l_2}(\Sigma)}{\partial \tilde{a}^{k_1}_{l_1}} - \frac{\partial\tilde{b}^{k_1}_{l_1}(\Sigma)}{\partial \tilde{a}^{k_2}_{l_2}} = 0$ which means there exists a holomorphic function $\mathcal{F}^{SL(n,\mathbb{C})} = \mathcal{F}^{SL(n,\mathbb{C})}(\{\tilde{a}^k_l\}, \{a_i\})$ on $\mathcal{B}^{SL(n,\mathbb{C})}$ such that
\begin{equation*}
    \tilde{b}^k_l = \frac{\partial \mathcal{F}^{SL(n,\mathbb{C})}}{\partial \tilde{a}^k_l}, \qquad b_i = \frac{\partial \mathcal{F}^{SL(n,\mathbb{C})}}{\partial a_i}.
\end{equation*}
We observe that $\tilde{b}^k_l = b^k_l - b^{k+1}_l$ and from $\frac{\partial}{\partial \tilde{a}^k_l} = \frac{\partial}{\partial a^k_l} - \frac{\partial}{\partial a^{k-1}_l}$, we conclude that if $\mathcal{F} = \mathcal{F}(\{a^k_l\}, \{a_i\})$ denotes the prepotential on $\mathcal{B}$ then $\mathcal{F}^{SL(n,\mathbb{C})} = \mathcal{F}|_{\mathcal{B}^{SL(n,\mathbb{C})}}$. 

\begin{remark}
The proof of the main theorem can be repeated in the case of $G = SL(n,\mathbb{C})$ with $\mathcal{B}^{SL(n,\mathbb{C})}, G^{SL(n,\mathbb{C})}_{\Sigma_0}, V^{SL(n,\mathbb{C})}_{\Sigma_0}$ and $\left(G^{SL(n,\mathbb{C})}_{\Sigma_0}\right)^\perp$ replacing $\mathcal{B}, G_{\Sigma_0}, V_{\Sigma_0}$ and $G^\perp_{\Sigma_0}$ respectively. Since we actually have $V^{SL(n,\mathbb{C})}_\Sigma = V_\Sigma$, the corresponding residue constraints Airy structure on $W^{Ram}_{Airy}$ will exactly be the same. As before, it will be convenient to pick the basis for $W^{Ram}_{Airy}$ to be $\{\tilde{\omega}^{k=1,\cdots,n}_{l=1,\cdots,g_C}, \tilde{\eta}^{k=1,\cdots,n}_{l=1,\cdots,g_C}, \omega_{i=1,2,3,\cdots}, \delta_{i=1,2,3,\cdots}\}$ where $\{\tilde{\omega}^k_l, \omega_i\}$ is a basis of $T_0L^{Ram}_{Airy}$, $\{\tilde{\eta}^k_l, \delta_i\}$ is a basis of $V^{SL(n,\mathbb{C})}_{\Sigma_0}$, $\{\omega_{i > g - ng_C}\}$ are locally defined, $\{\delta_{i > g-ng_C}\}$ spanned $G^\perp_{\Sigma_0}$ and 
\begin{equation*}
    \oint_{\tilde{A}^{k_1}_{l_1}}\tilde{\omega}^{k_2}_{l_2} = \delta^{k_1k_2}\delta_{l_1l_2},\qquad \oint_{\tilde{B}^{k_1}_{l_1}}\tilde{\omega}^{k_2}_{l_2} =: \tilde{\tau}^{k_1k_2}_{l_1l_2}(\Sigma_0) \qquad \oint_{A_i}\omega_j = \delta_{ij}, \qquad \oint_{B_i}\omega_j = \tau_{ij}(\Sigma_0).
\end{equation*}
Then we get
\begin{equation*}
    \frac{\partial^m\mathcal{F}^{SL(n,\mathbb{C})}}{\partial \tilde{a}^{k_1}_{l_1}\cdots \partial \tilde{a}^{k_m}_{l_m}} = -\left(\frac{i}{2\pi}\right)^{m-1}\oint_{p_1\in\tilde{B}^{k_1}_{l_1}}\cdots \oint_{p_m \in \tilde{B}^{k_m}_{l_m}}\omega_{0,m}(p_1,\cdots,p_m).
\end{equation*}
Note that the expansion $\omega_{g,m}(p_1,\cdots,p_m) = \sum_{k_1,\cdots,k_m}\sum_{l_1,\cdots, l_m} (S_{g,m})_{l_1,\cdots,l_m}^{k_1,\cdots,k_m}\tilde{\eta}^{k_1}_{l_1}\cdots\tilde{\eta}^{k_m}_{l_m}$ may contain the terms with $\tilde{\eta}^n_l$, i.e. the image of $S_{g,n} \in Sym_m(V_{\Sigma_0})$ under the quotient map may not be in $Sym_m(H^1(Prym(\Sigma_0, C), \mathbb{C}))$, those terms will vanish when evaluating against cycles from $H_1(Prym(\Sigma_0, C),\mathbb{C})$.
\end{remark}

\subsection{Quantum Airy structure from Higgs bundles}

    Recall, the base of the Hitchin system can be identified with the moduli space of deformations of $\Sigma$ inside the symplectic surface $X=T^* C$. 
    Let $\Sigma \rightarrow C$ be a simple ramified covering, with \(2n(n-1)(g_C-1) \) ramification points \(R\). As shown previously, there exists a symplectic vector space $W= \prod_{r \in R} W_{Airy}$.
    
    As we have seen in Section \ref{section:universal} the vector space $W$ can be decomposed as the direct sum $V \oplus V^*$, each with a corresponding Airy structure.
    
    Furthermore, this Airy structure can be quantised via deformation quantisation, as shown by \cite{KSoAir}, and described in Section~\ref{qairy}. This quantisation gives a wave function of the form 
    $$\psi_{\mathcal{L}}=\exp \left(S_0/\hb+\sum_{h \geq 1} S_h \hb^{h-1} \right).$$
    
    The resulting quantum Airy structure captures useful information about the special K\"ahler geometry of the moduli space $\cb^{reg}$.
    A prepotential for the special K\"ahler geometry is given by $F=\frac{1}{2} \sum_i z^i w_i$. The period matrix is given by $\tau_{ij}=\frac{\partial w_i}{\partial z^j}$, which is the same as $\frac{\partial^2 F}{\partial z^i \partial z^j}$.

    Recall that the Donagi-Markman cubic is given by
    $$c=\sum_{i,j,k} c_{ijk} dz^i \otimes dz^j \otimes dz^k,$$
    where 
    \[c_{ijk}=\frac{\partial \tau_{jk}}{\partial z^i}=\frac{\partial^3 F}{\partial z^i \partial z^j \partial z^k}.\]
    The connection between the Donagi-Markman cubic and the prepotential is studied in \cite{BHuSpe}. Using a version of Rauch variation formula it is proved that
    $$c_{ijk}=-\left(\frac{i}{2\pi}\right)^2 \int_{p_1 \in b_i} \int_{p_2 \in b_j} \int_{p_3 \in b_k} \omega_{0,3}(p_1,p_2,p_3).$$
    In the Airy structure picture, the prepotential corresponds to the genus zero part of the wavefunction \( \psi_{\mathcal{L}}\).


    \begin{proposition}
    Let $N,d$ be natural numbers. Consider the moduli space of Higgs bundles of rank $N$ and degree $d$ on a compact Riemann surface $C$ of genus $g_C>1$, together with the Hitchin system $f:\cm \to \cb$. For any point $b \in \cb^{reg}$ consider the associated Quantum Airy structure and the resulting wave function $\psi_{\mathcal{L}}$. Then
    $$\partial_{i_1} \partial_{i_2} \dots \partial _{i_{m-2}} \tau_{i_{m-1} i_m}(b)=-\left(\frac{i}{2\pi}\right)^{m-1} \int_{p_1 \in b_{i_1}} \dots \int_{p_m \in b_{i_m}} \omega_{0,m}(p_1,\dots,p_m),$$
    where $\omega_{0,m}$ are Eynard-Orantin invariants of the spectral curve $S_b$.
    \end{proposition}
    \begin{proof}
    This follows immediately from Theorem 1.
    \end{proof}


    In \cite[Theorem 1.3]{BHuSpe} it is also proved that for any point $b \in \cb^{reg}$,  they have the same relationship between the Taylor expansion of the prepotential and $b$-periods of the genus zero component $S_0$ of the wave function (although they used a different language). 
    
    It is mentioned that this formula is remarkable since the left hand side is related to geometry of a family of curves, while the right hand side only involves invariants of a single spectral curve. The results proved in this article show that this phenomenon occurs more generally. The same result occurs when the moduli space $\cb$ does not necessarily come from Higgs bundles. 
